Policy by Example: An Approach for Security Policy Specification

Policy specification for personal user data is a hard problem, as it depends on many factors that cannot be predetermined by system developers. Simultaneously, systems are increasingly relying on users to make security decisions. In this paper, we propose the approach of Policy by Example (PyBE) for specifying user-specific security policies. PyBE brings the benefits of the successful approach of programming by example (PBE) for program synthesis to the policy specification domain. In PyBE, users provide policy examples that specify if actions should be allowed or denied in certain scenarios. PyBE then predicts policy decisions for new scenarios. A key aspect of PyBE is its use of active learning to enable users to correct potential errors in their policy specification. To evaluate PyBE's effectiveness, we perform a feasibility study with expert users. Our study demonstrates that PyBE correctly predicts policies with 76% accuracy across all users, a significant improvement over naive approaches. Finally, we investigate the causes of inaccurate predictions to motivate directions for future research in this promising new domain.

==> acknowledgements.tex <==
% Jon Stallings.


==> applications.tex <==
\section{Applications}
\label{sec:applications}

Discuss the applications of our approach for solving the policy
specification problem in different domains (and for different kinds of
policies).

Does it make sense to have this section upfront after we describe our
overview?


==> background.tex <==
\section{Background - Nearest Neighbor Classification}
\label{sec:background}

A nearest neighbor (NN) search is the task of finding the {\em closest}
or most similar data point to a particular query point $q$, from a set
of points~\cite{mur12}. If used for classification, a 1NN classifier
predicts the class for a query point $q$ as the class of the closest
point in a set of already classified points $S$. A variant, kNN, may
instead consider the classes of k closest neighbors. Note that NN is an
unsupervised learning approach, i.e., the algorithm does not learn a
model, instead directly predicting based on the data points in the
training data. As a result, NN does not make any assumptions about the
probability distribution of data, making it workable even with small
datasets.

The most important aspect of learning with a kNN classifier is
determining the distance metric. The distance metric $\mu$ is a function
that computes the distance or similarity between two input data points.
Thus, the distance metric is the most crucial aspect for this approach.
In some scenarios, the metric may be obvious (e.g., computing the
distance among points in Euclidean space). For other scenarios, such as
when dealing with categorical data, a distance metric with desired
properties may need to be defined, as we do in
Section~\ref{sec:algorithm}.

\begin{comment}
\subsubsection{Breaking ties} Even when using 1-NN, a tie-breaking
strategy may be required for searches that result in more than one data
points at the closest distance, if the said points have different
classes. A naive strategy would be to pick one random data point from
the set of nearest neighbors. A more widely used strategy is to predict
the class of the majority data points. Such approaches often limit the
set size to an odd number, in order to have a certain majority. The
choice of the neighbor to exempt from the set of neighbors to achieve a
majority vote can be random, or made deterministic using some property
exclusive to the problem space.
\end{comment}


==> classification_results.tex <==
\subsection{Classification Results}
\label{sec:classifiers}

\begin{comment}
\begin{figure*}[t]
  \centering
  \captionsetup[subfloat]{captionskip=-1em}
  \subfloat[][Work Cloud
  policy]{\includegraphics[width=3in]{figs/plots/workcloud}\label{fig:workcloud}}
  \subfloat[][Work Email
  policy]{\includegraphics[width=3in]{figs/plots/workemailapp}\label{fig:workemailapp}}\\[-1em]
  \subfloat[][Personal Cloud
  policy]{\includegraphics[width=3in]{figs/plots/personalcloud}\label{fig:personalcloud}}
  \subfloat[][Personal Email
  policy]{\includegraphics[width=3in]{figs/plots/personalemailapp}\label{fig:personalemailapp}}\\[-1em]
  \subfloat[][Social
  policy]{\includegraphics[width=3in]{figs/plots/socialapp}\label{fig:socialapp}}
  \subfloat[][Work Wifi
  policy]{\includegraphics[width=3in]{figs/plots/workwifi}\label{fig:workwifi}}\\[-1em]
  \subfloat[][Home Wifi
  policy]{\includegraphics[width=3in]{figs/plots/homewifi}\label{fig:homewifi}}
  \caption{Accuracy of a decision tree across all responders, for each
  policy}
  \label{fig:policy_accuracy}
\end{figure*}

\begin{figure*}[t]
  \centering
  \captionsetup[subfloat]{captionskip=-1em}
  \subfloat[][Work Cloud
  policy]{\includegraphics[width=3in]{figs/plots/workcloud_cross}\label{fig:workcloud}}
  \subfloat[][Work Email
  policy]{\includegraphics[width=3in]{figs/plots/workemailapp_cross}\label{fig:workemailapp}}\\[-1em]
  \subfloat[][Personal Cloud
  policy]{\includegraphics[width=3in]{figs/plots/personalcloud_cross}\label{fig:personalcloud}}
  \subfloat[][Personal Email
  policy]{\includegraphics[width=3in]{figs/plots/personalemailapp_cross}\label{fig:personalemailapp}}\\[-1em]
  \subfloat[][Social
  policy]{\includegraphics[width=3in]{figs/plots/socialapp_cross}\label{fig:socialapp}}
  \subfloat[][Work Wifi
  policy]{\includegraphics[width=3in]{figs/plots/workwifi_cross}\label{fig:workwifi}}\\[-1em]
  \subfloat[][Home Wifi
  policy]{\includegraphics[width=3in]{figs/plots/homewifi_cross}\label{fig:homewifi}}
  \caption{Accuracy of a decision tree, for 10-fold cross validation, across all responders, for each
  policy}
  \label{fig:policy_accuracy}
\end{figure*}
\end{comment}



==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}


==> old/algorithm.tex <==
\section{The \pbes Algorithm}
\label{sec:algorithm}

This section describes our algorithm for predicting policy decisions,
and the active learning approach. As stated previously, distance between
policy examples is the distance between their scenarios. For simplicity,
however, our discussions are in terms of the policy example. 

Our policy examples (i.e., the scenarios) are Boolean functions over $n$
variables (i.e., tags), denoted by ${\cal B}_n$. However, we restrict
our attention to functions that are conjunctions of variables (e.g. $x_1
\wedge x_3 \wedge x_5$). Such a function $f$ can be represented as a set
$I(f) \subseteq \{ 1,2,\cdots,n \}$ (e.g., if $f = x_1 \wedge x_3 \wedge
x_5$, then $I(f) = \{ 1,3,5 \}$). Our examples belong to this
restricted class (denoted by ${\cal P}_n$). 

We had two requirements for the learning-algorithm to infer policies:
{\sf (I):} non-parametric (does not rely on models with a fixed set of
parameters).  {\sf (II):} easy explanation (easy to present to the
user how the policy was inferred). For this reason we chose a variant
of the {\it $k$ nearest neighbor (kNN)}
classifier~\cite{mur12}. A kNN algorithm simply ``looks at'' the
$k$ points in the training set that are nearest to the test input $x$,
counts how many members of each class are in the set, and returns that
empirical fraction as the estimate.

Recall that our goal is to label a policy example $p \in {\cal P}_n$
with the decision $1$ (i.e., {\sf allow}) or $0$ (i.e., {\sf deny}). We
are also given a set of examples along with known labels (i.e., policy
decisions).
%, say
%${\cal P}_l \subset {\cal P}_n$.  
Our algorithm is inspired by the kNN
algorithm and works as follows: given a new policy example $p \in {\cal
P}_n$ with an unknown label, we find the set of $k$ policy examples
$N(p) \; = \; \{ p_1,\cdots,p_k \}$ {\em closest} to $p$ according to
the metric $\mu$ (described in the next subsection) and then associate
the label to $p$ that corresponds to the majority labels of the policy
examples in $N(p)$. Our variant of kNN only considers examples at the
closest distance for inclusion in $N(p)$.  We describe how to address
situations where no majority exists in Section~\ref{sec:no-majority}.

%We adapt kNN for security policies, such that {\sf (1)} $N(p)$ only includes
%examples at the closest distance, and {\sf (2)} $k = |{\cal P}_l|$, since all
%labeled examples can be equally close to $p$.  
%Our intuition is that an
%algorithm for predicting security policies must be deterministic and
%rely on the closest neighbor(s), instead of an arbitrary value of $k$.

We use active learning to assist the user in correcting potential
labeling errors in the user's policy examples. When we find that certain
conditions are not true (e.g., the label of a policy example $q \in
{\cal P}_n$ is different from the majority label among its neighbors
$N(q)$), we recommend a change in the label~(e.g.,~change {\sf allow} to
{\sf deny}).  We now describe our metric $\mu$, its weighted form
$\mu_w$, and the active learning phase.

\subsection{The Metric}
\label{sec:metric}

Let $f$ and $g$ be two Boolean functions over $n$ variables
$x_1,x_2,\cdots,x_n$. A metric between $f$ and $g$ (denoted by
$\mu(f,g)$) can be defined as follows:
\[
1 - \frac{\sharp ( f \oplus g )}{2^n}
\]
Where $\oplus$ represents exclusive-or and $\sharp (h)$ is the number of
satisfying assignments of the Boolean function $h$. Recall that computing
the number of satisfying assignments of a Boolean function is a hard
problem ($\sharp$-P complete~\cite{ab09}). However, for our special case
(i.e. policies are conjunctions of variables) this metric is easy to
compute. Next we describe the metrics for the functions in the set
${\cal P}_n$. 

Consider two functions $f_1$ and $f_2$.  Let $[n] = \{1,2,\cdots,n\}$.
Consider three sets of indices $I_{1,2}$ (indices of variables neither in
$f_1$ nor $f_2$), $I^1_2$ (indices of variables in $f_1$ but not in
$f_2$) and $I^2_1$ (indices of variables in $f_2$ but not in $f_1$);
i.e.,  $I_{1,2} = [n] \setminus (I(f_1) \cup I(f_2))$, $I^1_2 = I(f_1)
\setminus I(f_2)$, and $I^2_1 = I(f_2) \setminus I(f_1)$.  An assignment
$\sigma$ is a Boolean vector of size $n$ of the form $\langle
b_1,b_2,\cdots,b_n \rangle$ and $f(\sigma)$ denotes the value of the
function $f$ for assignment $\sigma$.  

Consider an assignment $\sigma \; = \; \langle b_1,b_2,\cdots,b_n
\rangle$ such that $f_1(\sigma) = 1$ and $f_2 (\sigma) = 0$. Then for
all $i \in I(f_1)$, $b_i = 1$, and there should be at least one $i \in
I^2_1$ such that $b_i = 0$. For $i \in I_{1,2}$, $b_i$ can assume any
value. Consider all the indices in $I^2_1$. There should be at least one
$j \in I^2_1$, such that $b_j = 0$ (we want $f_2 (\sigma) = 0$).
Therefore, the number of satisfying assignments $\sigma$, such
that $f_1(\sigma) = 1$ and $f_2 (\sigma) = 0$ is
\[
2^{k_{1,2}} (2^{k_2} - 1)
\]
where $k_{1,2} = |I_{1,2}|$ and $k_2 = |I^2_1|$.
Explanation for the formula is as follows: all variables with indices
in the set $I_{1,2}$ can be given any value (resulting 
in the term $2^{k_{1,2}}$). All the variables with
indices in $I^2_1$ can be given any values as long as one of them 
is $0$, so  an assignment where all variables with indices in $I^2_1$
is assigned $1$ is excluded (this results in the term $2^{k_2}-1$).


A symmetric argument shows that the number of satisfying assignments
$\sigma$ such that $f_1 (\sigma) = 0$ and $f_2 (\sigma) = 1$ is 
\[
2^{k_{1,2}} (2^{k_1} - 1)
\]
where $k_{1,2} = |I_{1,2}|$ and $k_1 = |I^1_2|$.
Adding the two terms, we have that $\sharp (f_1 \oplus f_2)$ is
$2^{k_{1,2}} (2^{k_1}+2^{k_2}-2)$. Therefore, the metric $\mu
(f_1,f_2)$ in this case is:
\[
1 - \frac{2^{k_{1,2}} (2^{k_1}+2^{k_2}-2)}{2^n}
\]
where $k_{1,2} = |I_{1,2}|$, $k_1 = |I^1_2|$, and $k_2 =
|I^2_1|$. Intuitively, $k_1$ is the number of variables that
appear in $f_1$ but not in $f_2$, $k_2$ is the number of variables that
appear in $f_2$ but not in $f_1$, and $k_{1,2}$ is the number of
variables that appear in neither $f_1$ or $f_2$.  Let $k = n - k_{1,2}$,
which is the number of variables that appear in $f_1$ and $f_2$ (i.e.,
$k = |I(f_1) \cup I(f_2)|$ ). The metric $\mu (f_1,f_2)$  can 
be simplified as follows:
\[
\mu (f_1,f_2) = 1 - \frac{2^{k_1}+2^{k_2}-2}{2^k}
\]

Note that higher values of the metric indicate closeness.  
\begin{comment}
Further, recall Bob's example from Section~\ref{sec:overview}. In the
unweighted case, the distance metric (i.e., $\mu$) score between \{{\tt
Home,Document}\} and \{{\tt Document}\}, as well as between \{{\tt
Home,Document}\} and \{{\tt Home,Photo}\} is $0.75$.
\end{comment}

\subsection{The Weighted Metric} 
\label{sec:weighted-metric}

For security policies, some variables are more important than others;
e.g., recall the {\tt Home} tag from Bob's policy in
Section~\ref{sec:overview}. To incorporate the importance of variables
we introduce a weighted version of our metric.
As before, we will
consider a Boolean function over $n$ variables $x_1,x_2,\cdots,x_n$.
However, in this case we have two weights $w_i^0$ and $w_i^1$ associated
with each index $1 \leq i \leq n$. The weight associated with an
assignment $\sigma=\langle b_1,\cdots,b_n \rangle$ (denoted as
$w(\sigma)$) is
\[
\sum_{i=1}^n w_i^0 (1-b_i) + w_i^1 b_i \;.
\]
Given a set of Boolean assignments $S$, define $w(S)$ as 
$\sum_{\alpha \in S} w(\alpha)$ -- the sum of weights of
all assignments in $S$.  Given a Boolean function
$f$, $w(f)$ is the weight of the set of satisfying assignments 
of $f$. Using a simple 
recursive argument, the weight of all 
$2^n$ assignments $\{ 0,1 \}^n$ is:
\[
\prod_{i=1}^n (w_i^0+w_i^1)
\]

Given $n$ pair of weights $(w_1^0,w_1^1),\cdots,(w_n^0,w_n^1)$, a weighted metric between 
two Boolean functions $f$ and $g$ (denoted as $\mu_w(f,g)$) is defined as follows:
\[
1-\frac{w(f \oplus g)}{\prod_{i=1}^n (w_i^0+w_i^1)}
\]
Note that if for all $i$ we have $w_i^0=w_i^1=1$, we get the previous metric (i.e.,
the unweighted case).

As before, consider two Boolean functions $f_1$ and $f_2$ with index
sets $I(f_1)$ and $I(f_2)$. Let the index sets $I_2^1$ and $I_1^2$
be as defined before. Define the following three quantities:
\begin{eqnarray*}
z_1 & = & \prod_{i \in I_2^1} (w_i^0+w_i^1) \; - \;  \prod_{i \in I_2^1} w_i^0 \\
z_2 & = & \prod_{i \in I_1^2} (w_i^0+w_i^1) \; - \;  \prod_{i \in I_1^2} w_i^0 \\
z & = & \prod_{i \in I(f_1) \cup I(f_2) } (w_i^0+w_i^1) 
\end{eqnarray*}

The metric $\mu_w (f_1,f_2)$ can be defined as:
\[
\mu_w (f_1,f_2) = 1-\frac{z_1+z_2}{z}
\]
The argument is exactly same as before. The reader can check that for the unweighted
case (i.e. for all $i$ we have $w_i^0=w_i^1=1$) we get the previous metric back. 

\begin{comment}
Again, recall Bob's example from Section~\ref{sec:overview}, but for the
weighted case. That is, assume {\tt Home} has a weight $2$, whereas the
other tags all have the weight $1$. In the weighted case, the distance
metric (i.e., $\mu_w$) score between \{{\tt Home,Document}\} and \{{\tt
Document}\} is $0.67$, whereas that between \{{\tt Home,Document}\} and
\{{\tt Home,Photo}\} is $0.83$, i.e., the examples containing the
important tag {\tt Home} are nearer to each other.
\end{comment}


\myparagraph{Setting weights} Next we describe an algorithm to set
weights. Given a set of variables $V \; = \; \{x_1,\cdots,x_n\}$,
suppose we are given a partial order $\preceq$ on $V$ (e.g., $x_i
\preceq x_j$ means that $x_j$ is more ``important'' than $x_i$). Next we
construct a function $L: V \rightarrow [ n ]$ that assigns integers
between $1$ and $n$ to each variable in $V$ and has the property that
$x_i \preceq x_j$ and $j \not= i$ implies that $L(x_i) >
L(x_j)$.\footnote{ Such a function can be constructed by topologically
sorting a directed graph whose nodes are $V$ and there is an edge from
$x_j$ to $x_i$ ($j \not= i$) iff $x_i \preceq x_j$.} We can assign
higher weights $w_i^1$ to variables that have a lower value according to
the function $L$ and set all the weights $w_i^0$ to $1$. 
Note that it is not necessary to precisely define a mechanism for
assigning weights, as long as the ordering imposed by $L$ is preserved.

\subsection{Active Learning}
\label{sec:active-learning}

In an ideal scenario, users would provide accurate examples to \pbe.
However, as even expert users may not always be
accurate~\cite{yho+14,irc15}, we expect a small margin of error in
the policy decisions provided by the user; e.g., a typo resulting in 1
being accidentally marked as 0. We use active learning to find and
correct potentially incorrect labels, by asking users to relabel certain
chosen examples. The approach of relabeling samples to remove errors has
been shown to be effective even with non-experts by prior
work~\cite{spi08}.  

%The most important question in active learning is what query to pose to
%the oracle (i.e., the human annotator)~\cite{set09}. We use noise or
%inconsistency in the user's examples as an indicator of potential error,
%and a simply greedy algorithm to find what change to recommend to the
%user. 
%We use invariants on the nearest neighbor graph to quantify these
%inconsistencies. In the remainder of this section, we describe our
%approach for finding examples with potentially incorrect policy
%decisions, and our simply greedy algorithm for making recommendations
%to the user.

In our approach, the examples and their nearest neighbors are arranged
as a graph, which allows us to relabel existing examples in a systematic
manner if certain invariants on the graph are not true. In other words,
the graph we are about to describe gives us a systematic way to evaluate
the conditions that may be indicators of user error, and relabel
examples during the active learning phase.

Let $G = (V,E,L_V,L_E)$ be a $4$-tuple where $V \subseteq {\cal P}_n$ is
the set of labeled policy examples, $E\subseteq V \times V$ is the set
of edges, $L_V$ maps each vertex $v \in V$ with a label $1$ (signifying
{\sf allow}) and $0$ (signifying {\sf deny}), and $L_E$ labels each edge
$e \in E$ with a non-negative real value (i.e., $L_E (v,v')$ is $\mu (v,v')$,
which is the distance between the examples $v$ and $v'$).  The set of
neighbors $N(v)$ of a vertex $v \in V$ is the set $\{ v' \; | \; (v,v')
\in E \}$ and intuitively represents all the nearest-neighbors of the
policy $v$.
%As described before, we only consider neighbors at the
%closest distance in the nearest neighbor set $N(v)$ of a vertex $v$.
%Next we introduce two invariants on the graph $G$.

\noindent
{\bf (Inv-1): Majority label exists.} This invariant states that for all $v \in V$, 
its set of neighbors  $N(v)$ have a majority label 
(i.e,. more than $\frac{|N(v)|}{2}$ vertices in $N(v)$ have the same label
$L_V (v)$).

\noindent
{\bf (Inv-2): Agreement with the majority label.} This invariant states that
if invariant Inv-1 is true, then for every $v \in V$ its label
$L_V (v)$ agrees with the majority label of its neighbors $N(v)$.

Intuitively we want the graph $G$ corresponding to our policies to
satisfy invariants Inv-1 and Inv-2. If the graph $G$ violates either of
the invariants, then we recommend relabeling of examples to the user to
establish the two invariants.  

Figure~\ref{fig:invariants} shows instances of the graph for some vertex
$p$ that violate the invariants. In Figure~\ref{fig:invariant1}, there
is no majority label among $p's$ neighbors, which can be resolved by
relabeling either $q$ or $r$.  Further, in Figure~\ref{fig:invariant2},
the label on $p$ disagrees with the majority, which can be resolved by
relabeling $p$.   

\begin{figure}[t]
  \centering
  \subfloat[][$p$ violates Inv-1, i.e., no majority
  label]{\includegraphics[width=0.7in]{figs/invariant1}\label{fig:invariant1}}\qquad\qquad
  \subfloat[][$p$ violates Inv-2, i.e., disagrees with majority
  label]{\includegraphics[width=0.7in]{figs/invariant2}\label{fig:invariant2}}
  \caption{NN graph for vertex $p$, consisting of neighbors $q$ and $r$ at the closest distance $d$, violates Inv-1 and Inv-2.}
  \label{fig:invariants}
  \vspace{-1em}
\end{figure}

We use a simple greedy approach to recommend changes, briefly described
as follows:
%Our approach is to recommend the optimum label to change (i.e., $L_V
%(v_{opt})$), changing which results in a graph $G$ with the minimum
%violations.
%We briefly describe our algorithm as follows: 
Consider a function ${\cal V}(G)$ that counts the total violations of
both Inv-1 and Inv-2 in graph $G$. Further, consider a function ${\cal
C}(v,G)$ that measures the impact of a potential label change on
violations, i.e., returns the decrease in ${\cal V}(G)$ after a
temporary change in the label of $v$ (i.e., $L_V (v)$).  The
label change that causes the maximum decrease in ${\cal V}(G)$ is
optimal.  Therefore, at each iteration, we find the optimal vertex,
$v_{opt}$, by maximizing ${\cal C}(v,G)$ over all $v\in~V\setminus
V_{visited}$, where $V_{visited}$ is the set of all vertices that have
been recommended to the user previously. We add $v_{opt}$ to
$V_{visited}$, and recommend the user to change $L_V (v_{opt})$.  If the
user accepts, we change $L_V (v_{opt})$.  We reiterate until all the
vertices are visited or until there are no more violations.

Alternately, invariants may also be satisfied by generating additional
examples.
%First, we may generate examples to
%establish the invariant Inv-1. Assuming Inv-1 holds on the graph, we may
%then generate additional examples to establish the invariant Inv-2. 
As our current approach satisfies the objective of using noise for
finding potentially incorrect policy decisions, we did not explore
this alternative any further. 
%We propose \pbe as a
%general framework, into which a technique for recommending may be
%seamlessly incorporated in the future.


\subsection{Addressing no majority during prediction}
\label{sec:no-majority}
As described previously, we predict the label for a new example $p$ as
the majority label of its nearest neighbors $N(p)$. In case there
is no majority label, we use the following method to predict the label:

We eliminate the first neighbor that is not a {\em mutual} neighbor,
i.e., if there is a labeled example $q$ such that $q \in N(p)$ but $p
\notin N(q)$, we remove $q$ from $N(p)$, thereby converging on a
majority.  In case such elimination is not possible, i.e., if all
neighbors in $N(p)$ are mutual neighbors, we deny by default.  Our
method considers the value of the distance between neighbors to resolve
a tie, instead of randomly discarding one example (i.e., by only
considering only an odd number of examples in $N(p)$).  Our evaluation
demonstrates that \pbe is better than a baseline of random guessing. 

Finally, such cases of no majority were rarely seen during our
evaluation described in Section~\ref{sec:eval}; i.e.,  less than 6\%
test examples had no majority, and less than 3\% were denied by default.
However, as these results may be limited to our sample of study
participants, we do not make any general claims.


==> old/analysis_of_results.tex <==
\section{Analysis of Results}
\label{sec:analysis_of_results}

This paper is the first step towards our goal of a policy assistant. As
a result, our objective is not only to demonstrate a feasible approach,
but also to learn lessons for future work.  With this motivation, we
performed an in-depth study of our results to identify the general
causes of incorrect predictions. 

%\subsection{Causes of Incorrect Predictions}
We manually analyzed each of the 141 incorrectly predicted test
examples. For our analysis, we considered the following information
collected during our study: {\sf (1)} the justifications provided by the
participants for their policy decisions, {\sf (2)} the example(s) from
the specification dataset found nearest to the test example by our
algorithm, {\sf (3)} the weights set on each of the tags involved in the
test example, and {\sf (4)} all the examples in the specification
dataset that contain one or more of the tags included in the test
example.  The rest of this section describes the four causes of
incorrect predictions that we identified.  A detailed breakdown of the
causes across participants and policies is provided in
Table~\ref{tbl:incorrect}.  

\input{incorrect_tbl}

\subsection{Misconfigured Weights} 
We found that a majority of our incorrect predictions (79 out of 141, or
over 56\%) were caused because the weights set by the participants
contradicted their actual security preference. We confirmed our findings
using justifications from participants that clearly indicated the tag or
security preference that influenced their policy decision for a test
example. 

% \user{1}'s example.
\begin{table}[t]
\footnotesize
\centering
\caption{A subset of policy examples initially specified by \user{1},
which includes only those examples that contain {\tt Work}}
%\vspace{-0.5em}
\label{tbl:weight_cause}
\begin{tabular}{r|l|c}
  \Xhline{2\arrayrulewidth}
  {\bf No.} & {\bf Scenario}             & {\bf Policy Decision}\\
  \Xhline{2\arrayrulewidth}
  1 & \{Work, ScannedDocument\}   & deny  \\  
  2 & \{WhiteboardSnapshot, Work\} & deny\\
  3 & \{Work, BusinessCard\} & deny\\
  4 & \{Work, Audio\} & deny\\
  5 & \{Work, Postit\} & deny\\
  6 & \{Work\} & deny\\
  7 & \{Work, CalendarLink\} & deny\\
  8 & \{Work, Receipts\} & deny\\
  9 & \{Photos, Work\} & allow\\
  \Xhline{2\arrayrulewidth}
    \end{tabular} 
    \vspace{-1.5em}
\end{table} 

For instance, consider an incorrect prediction for \user{1} for the {\em
PersonalCloud} policy, where \pbe predicted the policy decision {\sf
allow} for \user{1}'s test example \{{\tt
WhiteboardSnapshot,Work,ScannedDocument}\}.  However, the user provided
the ground-truth decision of {\sf deny}, and with the quote ``{\em no
work data to personal cloud}''. That is, the tag {\tt Work} was
confidential and hence important to \user{1} with respect to the {\em
PersonalCloud} policy target.

Table~\ref{tbl:weight_cause} shows a subset of the initial examples
provided by \user{1}.  Observe that all of \user{1}'s examples that
contain {\tt Work} (except one) deny export to the {\em PersonalCloud}.
This leads us to conclude that \user{1} has consistently thought of {\tt
Work} as important with respect to the {\em PersonalCloud}.
However, this importance was not reflected in the weights, i.e.,
\user{1} mistakenly assigned {\tt Work} data a lower weight by ordering
it lower than personal data, as we saw previously in
Figure~\ref{fig:p1_order}. 

We investigated further by calculating numerical weights for each tag
involved in this incorrect prediction, using \user{1}'s weight orders
with the method described in Section~\ref{sec:weighted-metric}.  The tag
{\tt Work} had a low weight (i.e., 2), compared to other personal tags
(e.g., {\tt MedicalFacility}, weight 4). Therefore, rather than being
correctly identified as close to the work-related scanned document
scenario specified by \user{1} (i.e., {\tt Work, ScannedDocument}), the
test example was incorrectly identified as being close to the personal
policy examples \{{\tt MedicalFacility,ScannedDocument}\} and \{{\tt
WhiteboardSnapshot,MedicalFacility}\}, both of which allowed export to
the {\em PersonalCloud}.  Hence, the decision was incorrectly predicted
as {\sf allow}.

On raising the weight of {\tt Work} to 5 (i.e., above personal tags),
the test example was correctly found closer to \{{\tt
Work,ScannedDocument}\}, resulting in a correct prediction. Note that
this increase in weight is not arbitrary, but guided by evidence of the
user's security preferences. On correcting all misconfigured weights, we
manually confirmed that our overall accuracy rose to 89\%.  This
includes predictions for \user{2} and \user{5} for whom \pbe had the
lowest accuracy, i.e., most incorrect predictions for these users are
due to incorrect weights (which can be fixed), as shown in
Table~\ref{tbl:incorrect}.

Since misconfigured weights caused the maximum incorrect predictions (79
out of 141, or 56\%), we studied our data to find causes of incorrect
weights. We made two interesting observations, described as follows:


\emparagraph{Observation 1: Inaccurate predictions resulted from
participants only considering privacy preferences when setting weights.}
We observed that a large number of inaccuracies occurred when
participants did not take their security preferences for specific
security policy targets (e.g., {\em PersonalCloud}) into account while
setting weights, and set weights only based on their general privacy
preferences. However, since participants labeled examples based on their
security preferences, this resulted in incorrect predictions.

Recall that our participants were provided with the option of setting
different weight-group orders for different policy targets in
Section~\ref{sec:user_study}. However, all participants (except
\user{8}) set only a general order for all 5 policy targets, which only
accounted for the their privacy preferences. As a result,
higher-weighted personal tags (e.g., {\tt MedicalFacility}, {\tt Home})
had more influence on the policy decision, irrespective of the actual
policy target. This phenomenon caused false negatives for personal
policy targets such as {\em PersonalCloud} and {\em PersonalEmailApp},
since \pbe was forced to identify work-related test examples as closer
to personal examples, and hence predicted {\sf allow} instead of {\sf
deny} (e.g., as seen in \user{1}'s case previously).  Note that the
number of false positives for the {\em WorkCloud} and {\em WorkEmailApp}
policies was lower, as participants generally denied export for random
examples.

We confirmed that at least 26 incorrect predictions (out of 79 due to
weights) were false negatives in predicting the {\em PersonalCloud} and
{\em PersonalEmailApp} targets, which were directly caused by the
participant considering privacy preferences while setting weights, but
security preference (for work data) while labeling examples. 

\emparagraph{Observation 2: ``Important'' may not just mean
confidential.} In at least 14 of the test-examples incorrectly predicted
due to weights, participants wanted to set a high weight for a
non-confidential tag. From the justifications given by our participants
during testing, we realized that participants intended to declassify
data if a certain tag were present in the example. 

This was in complete contrast with the initial understanding of the
participants while setting weights, i.e., that confidential tags would
have high weights.  Thus, applying \pbe may require careful
consideration of what is ``important'', depending on the security goals
of the policy. We discuss the lesson learned from this observation in
Section~\ref{sec:lessons}.

%\myparagraph{2. Policy Change} 
\subsection{Policy Change} 
A significant minority (30 out of 141, or over 21\%) of our incorrect
predictions resulted from a change in the participants' policies, i.e.,
when participants explicitly disagreed with an earlier assumption they
made about their policy. 

\begin{comment}
Consider the test example shown in Listing~\ref{lst:cause_change}, where
\user{7}'s justification states that a {\tt Bookmark} created at home is
not safe for sharing to the personal cloud. However, an earlier example
shown in Listing~\ref{lst:cause_change} suggests that during the initial
policy specification, \user{7} chose to share a bookmark created at home
over the personal cloud. During our post-testing interview with
\user{7}, we confirmed that the participant's policy for the {\tt
Bookmark} and {\tt Photos} tags had changed recently. 
\end{comment}

Consider the example of \user{8}, whose policy has changed with respect
to the tag {\tt School}. During the initial policy specification, the
participant was employed off-campus, and hence assumed the tags {\tt
School} and {\tt Work} to have different meanings.  Therefore, the
policy decisions for school were often different than for work. Between
then and the testing phase, the participant changed jobs, and is now
employed with the school. As a result, during testing, the participant
provided similar policy decisions for work and school, and justified
with the quote ``{\em school is work}''. \user{8} admitted to this
change during the post-testing interview.  In all such cases, we
confirmed the policy change with evidence provided by participants in
their interviews or justifications.

Recall that the participants were provided with an opportunity to
indicate a change of mind during the manual review of examples described
in Section~\ref{sec:experiments}. All participants changed 35
decisions in total across policies. However, it is clear that
participants were unable to find all of their potential changes with a
manual review.  Thus, a policy assistant may need to account for the
participant's change of policy and prepare in advance, as we discuss in
Section~\ref{sec:future}.

%\myparagraph{3. Unconfirmed Policy Change}
\subsection{Unconfirmed Policy Change} For a small number of
incorrect predictions (15 out of 141, or about 11\%), we observed a
clear contradiction between the participant's examples during
specification and testing, but could not get a confirmation from the
participant.

Consider \user{8}'s test example \{{\tt SavedToDevice,Audio}\}, where
the ground truth label allows export for the {\em WorkCloud} policy.
However, all but one of \user{8}'s initially specified examples
containing {\tt SavedToDevice} or {\tt Audio} deny export to the work
cloud.  \user{8}'s justification stated that the participant had ``some
level of trust in the work cloud'', which neither confirms nor denies a
change of policy. Hence, we classify the cause for such cases as an
unconfirmed policy change. 

%\myparagraph{4. Tag Confusion} 
\subsection{Tag Confusion} 
The least number of errors (i.e., 12 out of
141, or about 8.5\%) were caused due to the ambiguity of some tags used
in our study.  The location or time-based tags (e.g., Home, Work,
Afterhours) were intended to indicate the location or time of creation
of different classes of data. As we did not place strict constraints on
our expert participants, our participants also created examples where
such tags could be used on their own (i.e., an example \{{\tt Home}\}
would mean data of an unknown type created at home).  Justifications
indicated that while participants had no trouble understanding the
examples they had created in their specifications, some random test
examples caused confusion.  Less than half of our participants faced
this problem, and for a few random text examples.

For example, \{{\tt Afterhours,Audio,Document}\} could mean Audio
created after hours, and added to a document whose origin is unknown, or
a document created after hours, and added to an audio recording whose
origin is unknown, and so on.  Participants indicated such confusion for
specific examples in their justifications during interviews.  We
describe a simple solution to this problem in Section~\ref{sec:lessons}.

Finally, we exclude five incorrectly predicted examples from \user{8}'s
test dataset from our categorization. For the examples (3 for {\em
PersonalEmailApp} and 2 for {\em WorkEmailApp}), the participant
suggested an inability to decide unless they knew the identity of the
email receiver, which gave us no information. We did not face this
situation with any other user or example.
%Further, the
%user was not able to express why they found the other examples workable
%for the same coarse-grained policies, but not the 5 specific examples.

\begin{comment}
In case of \user{5}, \pbes performs slightly worse in
predicting the {\em WorkCloud} and {\em WorkEmailApp} policies. This
inverse trend is mainly because many of the incorrectly predicted
examples result due to misconfigured weights of tags that can be
classified as personal data, but are generally considered to be
extremely sensitive, and must have higher weights than other personal
tags (e.g.,data collected at a Medical Facility).
\end{comment}


==> old/analysis_of_results_1.tex <==
\section{Analysis of Results}
\label{sec:analysis_of_results}

\pbe is the first step towards our vision of a policy assistant, and
one of our objectives is to learn lessons for future work.  With this
motivation, we performed an in-depth study of our results to identify
the general causes of incorrect predictions.

%\subsection{Causes of Incorrect Predictions}
We manually analyzed each of the 141 incorrectly predicted test
examples, using the following information
collected during our study: {\sf (1)} the justifications provided by the
participants for their decisions, {\sf (2)} the nearest neighbors of the
test example, {\sf (3)} the weights of the tags involved, and {\sf (4)}
all examples from the specification dataset that contain tags in common
with the test example.  The rest of this section describes the four
causes of incorrect predictions that we identified.  A detailed
breakdown of the causes across participants and policies is provided in
Table~\ref{tbl:incorrect} in Appendix~\ref{app:analysis}.  

%\input{incorrect_tbl}

\myparagraph{1. Misconfigured Weights} 
We found that a majority of our incorrect predictions (79 out of 141, or
over 56\%) were caused because the weights set by the participants
contradicted their actual security preferences. We confirmed our
findings using justifications from participants that clearly indicated
the tag or security preference that influenced their policy decision for
a test example. 

% \user{1}'s example.
\begin{table}[t]
\scriptsize
\centering
\caption{A subset of policy examples specified by \user{1},
which includes only those examples that contain {\tt Work}}
\vspace{-1em}
\label{tbl:weight_cause}
\begin{tabular}{r|l|c}
  \Xhline{2\arrayrulewidth}
  {\bf No.} & {\bf Scenario}             & {\bf Policy Decision}\\
  \Xhline{2\arrayrulewidth}
  1 & \{Work, ScannedDocument\}   & deny  \\  
  2 & \{WhiteboardSnapshot, Work\} & deny\\
  3 & \{Work, BusinessCard\} & deny\\
  4 & \{Work, Audio\} & deny\\
  5 & \{Work, Postit\} & deny\\
  6 & \{Work\} & deny\\
  7 & \{Work, CalendarLink\} & deny\\
  8 & \{Work, Receipts\} & deny\\
  9 & \{Photos, Work\} & allow\\
  \Xhline{2\arrayrulewidth}
    \end{tabular} 
    \vspace{-2em}
\end{table} 

For instance, consider an incorrect prediction for \user{1} for the {\em
PersonalCloud} policy, where \pbe predicted the policy decision {\sf
allow} for \user{1}'s test example \{{\footnotesize \tt
WhiteboardSnapshot,Work,ScannedDocument}\}.  The user provided the
ground-truth decision of {\sf deny}, and with the quote ``{\em no work
data to personal cloud}''. That is, the tag {\tt Work} was confidential
and hence important to \user{1} with respect to the {\em PersonalCloud}
policy target. This preference is also consistent for all but one of
\user{1}'s examples containing {\tt Work}, as shown in
Table~\ref{tbl:weight_cause}. Thus, we can conclude that \user{1} has
consistently considered {\tt Work} as important for the {\em
PersonalCloud}. However,  this importance was not reflected in the
weights, i.e., \user{1} mistakenly assigned {\tt Work} data a lower
weight (i.e., weight 2) by ordering it lower than personal data (i.e.,
weight 4), as we saw previously in Figure~\ref{fig:p1_order}. This
resulted in the test example being matched with personal examples (e.g.,
\{{\tt MedicalFacility,ScannedDocument}\}) that allowed export for
PersonalCloud.

\begin{comment}
Table~\ref{tbl:weight_cause} shows a subset of the initial examples
provided by \user{1}.  Observe that all of \user{1}'s examples that
contain {\tt Work} (except one) deny export to the {\em PersonalCloud}.
This leads us to conclude that \user{1} has consistently thought of {\tt
Work} as important with respect to the {\em PersonalCloud}.
However, this importance was not reflected in the weights, i.e.,
\user{1} mistakenly assigned {\tt Work} data a lower weight by ordering
it lower than personal data, as we saw previously in
Figure~\ref{fig:p1_order}. 
\end{comment}

\begin{comment}
We investigated further by calculating numerical weights for each tag
involved in this incorrect prediction, using \user{1}'s weight orders
with the method described in Section~\ref{sec:weighted-metric}.  The tag
{\tt Work} had a low weight (i.e., 2), compared to other personal tags
(e.g., {\tt MedicalFacility}, weight 4). Therefore, rather than being
correctly identified as close to the work-related scanned document
scenario specified by \user{1} (i.e., {\tt Work, ScannedDocument}), the
test example was incorrectly identified as being close to the personal
policy examples \{{\tt MedicalFacility,ScannedDocument}\} and \{{\tt
WhiteboardSnapshot,MedicalFacility}\}, both of which allowed export to
the {\em PersonalCloud}.  Hence, the decision was incorrectly predicted
as {\sf allow}.
\end{comment}

On raising the weight of {\tt Work} to 5 (i.e., above personal tags),
the test example was correctly found closer to \{{\tt
Work,ScannedDocument}\}, resulting in a correct prediction of {\sf
deny}. Note that this increase in weight is not arbitrary, but guided by
evidence of the user's security preferences. On correcting all
misconfigured weights, we manually confirmed that our overall accuracy
rose to 89\%.  This includes most predictions for \user{2} and \user{5}
for whom \pbe had the lowest accuracy.
%, i.e., most incorrect predictions for these users are due to incorrect
%weights (which can be fixed), as shown in Table~\ref{tbl:incorrect}.

Since misconfigured weights caused the maximum incorrect predictions (79
out of 141, or 56\%), we investigated further, and made two interesting
observations:

\emparagraph{Observation 1: Inaccurate predictions resulted from
participants only considering privacy preferences when setting weights.}
Recall that our participants were provided with the option of setting
different weight-group orders for different policy targets in
Section~\ref{sec:user_study}. All participants (except \user{8}) set
only a general order for all 5 policy targets, which only accounted for
the their privacy preferences. As a result, higher-weighted personal
tags (e.g., {\tt MedicalFacility}, {\tt Home}) had more influence on the
policy decision, irrespective of the actual policy target. However,
participants labeled examples based on their policy target-specific
security preferences (e.g., no work to {\em PersonlCloud}. This resulted
in incorrect predictions, as seen in \user{1}'s example previously. 

Note that this phenomenon occurs only because our tags are semantically
related to the policy targets (e.g., {\tt Work} to {\em WorkCloud}).  We
confirmed that at least 26 incorrect predictions (out of 79 due to
weights) were false negatives in predicting the {\em PersonalCloud} and
{\em PersonalEmailApp} targets, because participants considers privacy
for weights, and security for labeling.

\begin{comment}
Recall that our participants were provided with the option of setting
different weight-group orders for different policy targets in
Section~\ref{sec:user_study}. However, all participants (except
\user{8}) set only a general order for all 5 policy targets, which only
accounted for the their privacy preferences. As a result,
higher-weighted personal tags (e.g., {\tt MedicalFacility}, {\tt Home})
had more influence on the policy decision, irrespective of the actual
policy target. This phenomenon caused false negatives for personal
policy targets such as {\em PersonalCloud} and {\em PersonalEmailApp},
since \pbe was forced to identify work-related test examples as closer
to personal examples, and hence predicted {\sf allow} instead of {\sf
deny} (e.g., as seen in \user{1}'s case previously).  Note that the
number of false positives for the {\em WorkCloud} and {\em WorkEmailApp}
policies was lower, as participants generally denied export for random
examples.

We confirmed that at least 26 incorrect predictions (out of 79 due to
weights) were false negatives in predicting the {\em PersonalCloud} and
{\em PersonalEmailApp} targets, which were directly caused by the
participant considering privacy preferences while setting weights, but
security preference (for work data) while labeling examples. 

\end{comment}
\emparagraph{Observation 2: ``Important'' may not just mean
confidential.} In at least 14 of the test-examples incorrectly predicted
due to weights, participants wanted to set a high weight for a
non-confidential tag, i.e., to declassify data if a certain tag were
present in the scenario. This was in complete contrast with the initial
understanding of the participants while setting weights, i.e., that
confidential tags would have high weights. 

%From the justifications given by our participants
%during testing, we realized that participants intended to declassify
%data if a certain tag were present in the example. 

\begin{comment}
This was in complete contrast with the initial understanding of the
participants while setting weights, i.e., that confidential tags would
have high weights.  Thus, applying \pbe may require careful
consideration of what is ``important'', depending on the security goals
of the policy. We discuss the lesson learned from this observation in
Section~\ref{sec:lessons}.
\end{comment}

\myparagraph{2. Policy Change} 
A significant minority (30 out of 141, or over 21\%) of our incorrect
predictions resulted from a change in the participants' policies, i.e.,
when participants explicitly disagreed with an earlier assumption. 

For example,  \user{8}'s policy changed for the tag {\tt School}. During
the initial specification, \user{8} assumed {\tt School} and {\tt Work}
to be different due to off-campus employment. However, before testing,
\user{8} started working at the school, which resulted in similar
decisions for {\tt School} and {\tt Work}. \user{8} admitted to this
change during the post-testing interview. All cases in this category
were similarly confirmed.

%Recall that the participants were provided with an opportunity to
%indicate a change of mind during the manual review of examples  described
%in Section~\ref{sec:experiments}. All participants changed 35
%decisions in total across policies. However, it is clear that
%participants were unable to find all of their potential changes with a
%manual review.  

\myparagraph{3. Unconfirmed Policy Change} For a small number of
incorrect predictions (15 out of 141, or about 11\%), we observed a
clear contradiction between the participant's examples during
specification and testing, but could not get a confirmation from the
participant. For example, for \user{8}'s test example \{{\tt
SavedToDevice,Audio}\}, the ground truth label allows export for the
{\em WorkCloud} policy, but all except one of \user{8}'s initially
specified examples containing {\tt SavedToDevice} or {\tt Audio} deny
export to the {\em WorkCloud}. Without additional information, we
classify such contradictions as unconfirmed policy changes.

%Consider \user{8}'s test example \{{\tt SavedToDevice,Audio}\}, where
%the ground truth label allows export for the {\em WorkCloud} policy.
%However, all but one of \user{8}'s initially specified examples
%containing {\tt SavedToDevice} or {\tt Audio} deny export to the work
%cloud.  \user{8}'s justification stated that the participant had ``some
%level of trust in the work cloud'', which neither confirms nor denies a
%change of policy. Hence, we classify the cause for such cases as an
%unconfirmed policy change. 


%\myparagraph{4. Tag Confusion} 
\myparagraph{4. Tag Confusion} 
The least number of errors (i.e., 12 out of
141, or about 8.5\%) were caused due to the ambiguity of some tags used
in our study.  The location or time-based tags (e.g., Home, Work,
Afterhours) were intended to indicate the location or time of creation
of different classes of data. However, as we did not place strict
constraints on our expert participants, our participants also created
examples where such tags could be used by themselves (i.e., the scenario
\{{\tt Home}\} would mean data of an unknown type created at home).
Justifications indicated that while participants had no trouble
understanding the examples they had created,
some random test examples caused confusion.  Less than half of our
participants faced this problem, and for a few random text examples.
For example, \{{\tt Afterhours,Audio,Document}\} could mean Audio
created after hours, and added to a document whose origin is unknown, or
a document created after hours, and added to an audio recording whose
origin is unknown, and so on.  

Finally, we exclude five incorrectly predicted examples from \user{8}'s
test dataset from our categorization. For the examples (3 for {\em
PersonalEmailApp} and 2 for {\em WorkEmailApp}), the participant
suggested an inability to decide unless they knew the identity of the
email receiver, which gave us no information. We did not face this
situation with any other user or example.
%Further, the
%user was not able to express why they found the other examples workable
%for the same coarse-grained policies, but not the 5 specific examples.

\begin{comment}
In case of \user{5}, \pbes performs slightly worse in
predicting the {\em WorkCloud} and {\em WorkEmailApp} policies. This
inverse trend is mainly because many of the incorrectly predicted
examples result due to misconfigured weights of tags that can be
classified as personal data, but are generally considered to be
extremely sensitive, and must have higher weights than other personal
tags (e.g.,data collected at a Medical Facility).
\end{comment}


==> old/conc.tex <==
\section{Conclusion} \label{sec:conc}

We introduced the paradigm of Policy by Example (\pbe) for user-specific
policy specification. \pbe enables users to express data-use
scenarios in policy examples, and predicts policy decisions for new
scenarios. A salient aspect of \pbe is its active learning approach for
engaging users in finding and potentially incorrect policy decisions in
their examples.  In our feasibility study with expert users, \pbe
demonstrated over 76\% prediction accuracy, and better average
performance than a baseline and a naive approach.  A significant finding
was that \pbe's interactive approach was five times as effective as a
manual review in finding errors.  Finally, we analyzed our incorrect
predictions and learned lessons that motivate future
research in this promising new domain.


==> old/experiments.tex <==
\subsection{Data Collection}
\label{sec:user_study}

This section describes the approach used for collecting the policy
examples and weights from participants, the scripts for which can be
found in Appendix~\ref{app:examples_script} and
Appendix~\ref{app:weights_script} respectively.
%\bibnote{citation for semi-structured interviews}

\myparagraph{1. Collecting Policy Examples} Participants were provided
with our predefined tags, but were also allowed to create their own
tags. Participants were instructed that they could combine tags into
complex scenarios for creating examples.  We placed no constraint on the
number of example scenarios each participant could provide. For each
scenario, participants were required to label policy decisions for the 5
targets described previously in Table~\ref{tbl:policy}.  Note
that we collected labels for two more targets, but discarded them
before testing to reduce user fatigue.  
%The script for this task is provided in
%Appendix~\ref{app:examples_script}.

A preliminary analysis of the examples collected from our participants
let to two interesting observations: {\sf (1)} Our participants created
a total of 31 unique tags, out of which about 58\% (or 23) were specific
to individual participants, while only 7 tags were commonly used by all
in their examples, and {\sf (2)} Out of the 246 example scenarios
collected across participants, over 76\% were specific to individual
participants, and only 7 were common among all 8 participants. These
observations indicate that relevant {\em data-use scenarios may be
unique to the individual, even among student researchers from the same
research lab}, further motivating our research into generating
user-specific policies for user-specific data.

\begin{comment}
Note that although we allowed our participants to create tags to get complex
security policies, non-experts may not need to create tags under
ordinary circumstances.  We discuss ideas for collecting policy examples
from non-experts in Section~\ref{sec:future}. 
\end{comment}

% Some stats for use in the paper.
%Total users=8, 
%Total examples provided=246, 
%Average examples provided=30.75, 
%Total (non-unique) tags used=112, 
%Average tags used=14.00.

\myparagraph{2. Obtaining Weights} On average,  each
participant used about 14 unique tags in their examples. As ordering a
large number of tags can be tiring, we categorized  tags into semantic
groups. The participants were provided with this semantic grouping, and
were {\sf (1)} first allowed to customize group memberships of tags as
per their understanding (e.g., Figure~\ref{fig:tag_groups} in
Appendix~\ref{app:weights_script}), and then {\sf (2)} instructed to
provide a partial order over the groups in a spreadsheet, as seen in the
partial order created by \user{1} in Figure~\ref{fig:p1_order}.
Participants were provided with a basic partial order generated by the
authors, and could start from scratch, or customize the order we
provided to generate their own custom order.  
%Scripts for both tasks can be found in
%Appendix~\ref{app:weights_script}.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.2in]{figs/response_order}
    \vspace{-0.5em}
    \caption{Screenshot of \user{1}'s ordering of tag groups.}
    \label{fig:p1_order}
    \vspace{-1em}
\end{figure}

We confirmed each partial order relation by reading it out to the user.
For example, for \user{1}, we asked if ``Personal data is more important
than Work data'', to confirm {\tt Work;Personal} shown in
Figure~\ref{fig:p1_order}. The orders were then used to generate weights
as described in Section~\ref{sec:weighted-metric}.

Further, participants were informed that they could provide different
partial orders for different policies, but most participants chose to
keep a single general order.  We describe the impact of
this decision in Section~\ref{sec:analysis_of_results}.  

\begin{comment}
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,float=tp,caption={Participant-generated
  partial order on tag groups.},belowcaptionskip=-6mm,label=lst:context-ordering,emph={RULE,GROUPS},emphstyle=\bfseries]
# RULE: If i<-j, then j is more important than i
# GROUPS: {Finance,Medical,Work,Personal,Documents,History,Notes,Recordings,Todo}
Medical<-Finance
Work<-Medical
\end{lstlisting}
\end{comment}

\subsection{Experiments}
\label{sec:experiments}
%% IDENTIFYING AND RESOLVING USER ERRORS
This section describes the experiments used for identifying user errors
and testing prediction for randomly generated scenarios, the scripts for
which can be found in Appendix~\ref{app:review_script} and
Appendix~\ref{app:testing_script} respectively.

\myparagraph{1. Identifying Errors}
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,float=tp,caption={A
  suggestion made 
  by the \pbes algorithm during the interactive review
  process.},belowcaptionskip=-6mm,label=lst:suggestion,emph={Suggestion},emphstyle=\bfseries]
Suggestion: For {Note}, WorkCloud = DENY. Agree?(y/n)
\end{lstlisting}
%
The review of examples was carried out 3 months after the initial
specification, as most participants were unavailable over the summer
break.  
%The objective of  review was to give participants an
%opportunity to correct their examples before testing, and to evaluate
%the effectiveness of our active learning approach.
We performed a two-step experiment to help participants identify and
correct errors in their policy decisions.  
%Scripts for these tasks can be found in
%Appendix~\ref{app:review_script}.

First, participants performed a manual review of their initial
specification. Participants were provided with a spreadsheet containing
their policy examples (one sheet per policy target), and could change
any policy decision they desired.  For each update, participants were
instructed to indicate a cause to justify the change (e.g., correcting
an error, change of mind, inability to decide). Finally, participants
provided a justification for each change (e.g., ``Work is
confidential''), providing the helpful context for analyzing the results
(Section~\ref{sec:analysis_of_results}).

After the manual review, we performed a \pbe-assisted review using the
approach described in Section~\ref{sec:active-learning}. We treat each
participant-policy combination as a separate policy specification
problem; hence, a separate review was performed for each such case
(i.e., 8 users and 5 policies make 40 total cases). As we used the
changed examples from the manual review; any errors discovered using
this approach were additional. Our algorithm presented the participant
with a series of suggestions (i.e., examples with corrected policy
decisions, as shown in Listing~\ref{lst:suggestion}).  If the
participant accepted the suggestion, we confirmed with the participant
that the original decision was in error, and recorded it as an error
found by \pbe.  If the participant rejected, we asked for a short
justification to understand the participant's policy preferences. We
stopped at 15 suggestions for each participant-policy case to limit
fatigue.  

%% TESTING FOR ACCURACY
\myparagraph{2. Testing with Random Examples}
For each participant, we randomly generated $n/2$ new policy scenarios,
where $n$ was the number of scenarios initially provided by the
participant.  The random scenarios were created
with the tags used in the participant's initial examples.  The intuition
is that the tags provided by the participant are relevant to the
participant, hence scenarios composed of them must be relevant as
well. To mitigate labeling fatigue, the random scenarios included at
most 3 tags. 
%The  experiment script is provided in Appendix~\ref{app:testing_script}.
%We take two decisions to limit user fatigue: 1) we limit the random
%examples to include at most 3 tags, and 2) we
%consider only the first 5 policies, and exclude the {\em Workwifi} and
%{\em Homewifi} policies from the testing set.  

Participants provided the ground truth policy decisions for their
test scenarios, for each of the five policy targets.  Apart from
indicating ``Allow'' or ``Deny'', participants were also provided the
``I don't know'', in which case we substituted the scenario with another
random test scenario.  We predicted the policy decision for each test
scenario using our algorithm. We then asked participants to confirm
their decisions for incorrect predictions, provide short justifications,
and conducted short, informal interviews that helped us gain insight
into the decisions.
\begin{comment}
For incorrect predictions, participants
were asked to confirm their decisions and provide short justifications.
After concluding the testing experiment, we conducted a short informal
interview to gain insight into the participant's decisions,
which helped us analyze our results in
Section~\ref{sec:analysis_of_results}.
\end{comment}


==> old/experiments_1.tex <==
\vspace{-1em}
\subsection{Data Collection}
\label{sec:user_study}
\vspace{-0.5em}

This section describes the approach used for collecting the policy
examples and weights from participants, the scripts for which can be
found in Appendix~\ref{app:examples_script} and
Appendix~\ref{app:weights_script} respectively.
%\bibnote{citation for semi-structured interviews}

\myparagraph{1. Collecting Policy Examples} Participants were provided
with our predefined tags, but were also allowed to create their own
tags. Participants were instructed that they could combine tags into
complex scenarios for creating examples.  We placed no constraint on the
number of example scenarios each participant could provide. For each
scenario, participants were required to label policy decisions for the 5
targets described previously in Table~\ref{tbl:policy}.  Note
that we collected labels for two more targets, but discarded them
before testing to reduce user fatigue.  
%The script for this task is provided in
%Appendix~\ref{app:examples_script}.

A preliminary analysis of the examples collected from our participants
let to two interesting observations: {\sf (1)} Our participants created
a total of 31 unique tags, out of which about 58\% (or 23) were specific
to individual participants, while only 7 tags were commonly used by all
in their examples, and {\sf (2)} Out of the 246 example scenarios
collected across participants, over 76\% were specific to individual
participants, and only 7 were common among all 8 participants. These
observations indicate that relevant {\em data-use scenarios may be
unique to the individual, even among student researchers from the same
research lab}, further motivating our research into generating
user-specific policies for user-specific data.

\begin{comment}
Note that although we allowed our participants to create tags to get complex
security policies, non-experts may not need to create tags under
ordinary circumstances.  We discuss ideas for collecting policy examples
from non-exerts in Section~\ref{sec:future}. 
\end{comment}

% Some stats for use in the paper.
%Total users=8, 
%Total examples provided=246, 
%Average examples provided=30.75, 
%Total (non-unique) tags used=112, 
%Average tags used=14.00.

\myparagraph{2. Obtaining Weights} On average,  each participant used
about 14 unique tags in their examples. As ordering a large number of
tags can be tiring, we categorized  tags into semantic groups. The
participants were provided with this semantic grouping, and were {\sf
(1)} first allowed to customize group memberships of tags as per their
understanding (e.g., Figure~\ref{fig:tag_groups} in
Appendix~\ref{app:weights_script}), and then {\sf (2)} instructed to
provide a partial order over the groups in a spreadsheet (e.g.,
\user{1}'s partial order in Figure~\ref{fig:p1_order}).  Participants
were provided with a basic partial order generated by the authors, and
could start from scratch, or customize the order we provided to generate
their own custom order.  We confirmed each partial order relation by
reading it out to the user; e.g., by asking if ``j is more important
than i'' to confirm {\tt i;j}. We then transformed the orders to weights
using the approach described in Section~\ref{sec:weighted-metric}.
%Scripts for both tasks can be found in
%Appendix~\ref{app:weights_script}.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.2in]{figs/response_order}
    \vspace{-0.5em}
    \caption{Screenshot of \user{1}'s ordering of tag groups.}
    \label{fig:p1_order}
    \vspace{-1em}
\end{figure}

%We confirmed each partial order relation by reading it out to the user.
%For example, for \user{1}, we asked if ``Personal data is more important
%than Work data'', to confirm {\tt Work;Personal} shown in
%Figure~\ref{fig:p1_order}. The orders were then used to generate weights
%as described in Section~\ref{sec:weighted-metric}.

Further, participants were informed that they could provide different
partial orders for different policies, but most participants chose to
keep a single general order.  We describe the impact of
this decision in Section~\ref{sec:analysis_of_results}.  

\begin{comment}
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,float=tp,caption={Participant-generated
  partial order on tag groups.},belowcaptionskip=-6mm,label=lst:context-ordering,emph={RULE,GROUPS},emphstyle=\bfseries]
# RULE: If i<-j, then j is more important than i
# GROUPS: {Finance,Medical,Work,Personal,Documents,History,Notes,Recordings,Todo}
Medical<-Finance
Work<-Medical
\end{lstlisting}
\end{comment}
\vspace{-1em}
\subsection{Experiments}
\label{sec:experiments}
\vspace{-0.5em}
%% IDENTIFYING AND RESOLVING USER ERRORS
This section describes the experiments used for identifying user errors
and testing prediction for randomly generated scenarios, the scripts for
which can be found in Appendix~\ref{app:review_script} and
Appendix~\ref{app:testing_script} respectively.

\myparagraph{1. Identifying Errors}
\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,float=tp,caption={A
  suggestion made 
  by the \pbes algorithm during the interactive review
  process.},belowcaptionskip=-6mm,label=lst:suggestion,emph={Suggestion},emphstyle=\bfseries]
Suggestion: For {Note}, WorkCloud = DENY. Agree?(y/n)
\end{lstlisting}
%
The review of examples was carried out 3 months after the initial
specification, as most participants were unavailable over the summer
break.  
%The objective of  review was to give participants an
%opportunity to correct their examples before testing, and to evaluate
%the effectiveness of our active learning approach.
We performed a two-step experiment to help participants identify and
correct errors in their policy decisions.  
%Scripts for these tasks can be found in
%Appendix~\ref{app:review_script}.

First, participants performed a manual review of their initial
specification. Participants were provided with a spreadsheet containing
their policy examples (one sheet per policy target), and could change
any policy decision they desired.  For each update, participants were
instructed to indicate a cause to justify the change (e.g., correcting
an error, change of mind, inability to decide). Finally, participants
provided a justification for each change (e.g., ``Work is
confidential''), providing the helpful context for analyzing the results
(Section~\ref{sec:analysis_of_results}).

After the manual review, we performed a \pbe-assisted review using the
approach described in Section~\ref{sec:active-learning}. We treat each
participant-policy combination as a separate policy specification
problem; hence, a separate review was performed for each such case
(i.e., 8 users and 5 policies make 40 total cases). As we used the
changed examples from the manual review; any errors discovered using
this approach were additional. Our algorithm presented the participant
with a series of suggestions (i.e., examples with corrected policy
decisions, as shown in Listing~\ref{lst:suggestion}).  If the
participant accepted the suggestion, we confirmed with the participant
that the original decision was in error, and recorded it as an error
found by \pbe.  If the participant rejected, we asked for a short
justification to understand the participant's policy preferences. We
stopped at 15 suggestions for each participant-policy case to limit
fatigue.  

%% TESTING FOR ACCURACY
\myparagraph{2. Testing with Random Examples}
For each participant, we randomly generated $n/2$ new policy scenarios,
where $n$ was the number of scenarios initially provided by the
participant.  The random scenarios were created
with the tags used in the participant's initial examples.  The intuition
is that the tags provided by the participant are relevant to the
participant, hence scenarios composed of them must be relevant as
well. To mitigate labeling fatigue, the random scenarios included at
most 3 tags. 
%The  experiment script is provided in Appendix~\ref{app:testing_script}.
%We take two decisions to limit user fatigue: 1) we limit the random
%examples to include at most 3 tags, and 2) we
%consider only the first 5 policies, and exclude the {\em Workwifi} and
%{\em Homewifi} policies from the testing set.  

Participants provided the ground truth policy decisions for their
test scenarios, for each of the five policy targets.  Apart from
indicating ``Allow'' or ``Deny'', participants were also provided the
``I don't know'', in which case we substituted the scenario with another
random test scenario.  We predicted the policy decision for each test
scenario using our algorithm. We then asked participants to confirm
their decisions for incorrect predictions, provide short justifications,
and conducted short, informal interviews that helped us gain insight
into the decisions.


==> old/future.tex <==
\section{Future Directions}
\label{sec:future}

Our evaluation of \pbe demonstrates feasibility with expert users, and
shows promise for further exploration in this area.  In this section, we
discuss two future research directions, namely {\sf (1)} adapting \pbe
for non-experts and {\sf (2)} adapting to change in policy decisions.

\subsection{Adapting \pbe for non-experts}
Measuring the usability of \pbe with non-experts is a natural direction for
future research. We make the following recommendations for tasks that
may be performed differently for non-experts.

\subsubsection{Collecting examples} To ease the burden of creating tags,
non-experts may be provided with a large and diverse collection of tags
(e.g., the 40 tags obtained in our study) as a baseline for specifying
examples. Further, user-friendly user interfaces may be required for non
experts. We are actively considering the concept of ``interactive
dropdowns'' to collect examples~\cite{jkkg10a,jkkg10b}.
%Providing initial tags may also motivate the user to create new tags. 

Further, non-experts cannot be expected to specify examples without a user
interface as expert users did in Section~\ref{sec:user_study}. A
challenge for future work is to acquire policy examples without
burdening the user. We are actively considering the approach of using
``interactive dropdowns'' to collect examples, as described in
prior work on usable policy authoring~\cite{jkkg10a,jkkg10b}.

\subsubsection{Collecting Weights} Collecting weights from non-experts
while reducing user-burden is another challenge for future work.  Our
approach for setting weights (described in
Section~\ref{sec:weighted-metric}) allows users to describe relative tag
weights in terms of partial order relations on tags. To improve the
usability of this approach we are considering using visual ``sliders''
for weight collection, which will allow users to easily select more
precise weights.

Additionally, incorporating \pbe into an existing system may require
careful consideration of run-time overrides. That is, power-users may
want to override policy decisions predicted by \pbe during runtime, or
provide feedback. The advantage of incorporating such overriding
mechanism is that the user's correct decision may be added to the user's
policy examples to improve future predictions. The challenge is of
indicating to the user that a prediction has been made, while causing
minimum interference with the user's task.

\begin{comment}
Minor challenges:
3. Conflict resolution: While we collected the specification dataset only
once for our study, in reality, the user may modify their specification
whenever they please. The conflict-resolution routine may have to
execute whenever the dataset is modified. For usability, we may need to
remember user's response to recommendations between subsequent
executions.

While the following does not directly concern \pbe, it still is an
important point:

4. Runtime predictions: Depending on user preference, users may want to
override certain decisions at runtime. The enforcement system must then
ask the user to update the policy specification.
\end{comment}

\subsection{Adapting to Change in Policy Decisions}
Section~\ref{sec:analysis_of_results} shows that over 21\%
incorrect predictions were due to change in the participant's policy.
Future research may be directed at solving the problem of detecting
potential change in policy from current examples. Our intuition is that
while detecting change in some cases may be impossible without external
input (e.g., change in policy for {\tt Work} data due to loss of
employment), there is potential in evaluating solutions to this
problem for other cases. We describe three challenges in this area, as
follows: 
\subsubsection{Identifying the causes of policy change} Identifying and
studying the causes of change in security policy is a precondition for
demarcating the line between policy changes that can and cannot be
addressed with machine learning. A longitudinal user study may need
to be performed to find if users change policies frequently, and to
identify the causes, as prior work has done for file access control
policies~\cite{sg09}.
\subsubsection{Identifying the time of policy change} Identifying when a
policy change happens is hard without any input from the user. One
approach to address this challenge is to encourage users to report
policy changes. Future work may take lessons from persuasive
technologies that change user behavior and motivate users to participate
in the desired activity~\cite{cml09,mc12,pgb+10}.
\subsubsection{Identifying the example(s) to change} Instead of waiting
for the user to indicate change, the learner may be able to use existing
information (e.g., tag weights, frequency in examples) to detect what
example or tag may be subject to change. Our intuition is that
strategies used for cache replacement (e.g., least recently used or
LRU~\cite{sj94}) may be applicable to this domain, at least as a
starting point.

Finally, active learning may also be used to suggest new examples to the
user, which is not the focus of this paper. Instead, the focus of \pbe
is on predicting the user's policy decisions for new scenarios.
Generating new examples lies in the broader scope for future work.



==> old/future_1.tex <==
\vspace{-1em}
\section{Future Directions}
\label{sec:future}
\vspace{-0.5em}

Our evaluation of \pbe demonstrates feasibility, and shows promise for
further exploration in this area.  We now discuss two future directions,
namely {\sf (1)} adapting \pbe for non-experts and {\sf (2)} adapting to
change.

\myparagraph{Adapting \pbe for non-experts}
Measuring the usability of \pbe with non-experts is a natural direction
for future research. Additionally, we make the following recommendations
for tasks that may be performed differently for non-experts.

\emparagraph{1. Collecting examples:} To ease the burden of creating
tags, non-experts may be provided with a large and diverse collection of
tags (e.g., the 40 tags obtained in our study) as a baseline for
specifying examples. Further, usable interfaces may be considered for
non experts (e.g., ``interactive dropdowns''~\cite{jkkg10a,jkkg10b} to
collect examples).
%Providing initial tags may also motivate the user to create new tags. 

\emparagraph{2. Collecting Weights:} Collecting weights from non-experts
is another challenge for future work. Future work may consider using
visual ``sliders'' for weight collection, for precise and usable weight
assignments.

\emparagraph{3. System Deployment:} \pbe may be incorporated into
existing systems which protect user data from disclosure to the network
(e.g., Weir~\cite{naej16} and Aquifer~\cite{ne13}). On such systems,
users may want to override policy predictions by \pbe at runtime, or
provide feedback, requiring a trusted path between the user and
\pbe.  A feedback mechanism may also improve future predictions.

%Incorporating \pbe such
%systems may require
%careful consideration of run-time overrides. Power-users may
%want to override policy decisions predicted by \pbe during runtime, or
%provide feedback. The advantage of incorporating such overriding
%mechanism is that the user's correct decision may be added to the user's
%policy examples to improve future predictions. The challenge is of
%indicating to the user that a prediction has been made, while causing
%minimum interference with the user's task.

\begin{comment}
Minor challenges:
3. Conflict resolution: While we collected the specification dataset only
once for our study, in reality, the user may modify their specification
whenever they please. The conflict-resolution routine may have to
execute whenever the dataset is modified. For usability, we may need to
remember user's response to recommendations between subsequent
executions.

While the following does not directly concern \pbe, it still is an
important point:

4. Runtime predictions: Depending on user preference, users may want to
override certain decisions at runtime. The enforcement system must then
ask the user to update the policy specification.
\end{comment}

\myparagraph{Adapting to Change}
Future research may be directed at detecting potential change in the
policy from current examples. While detecting
change in some cases may be impossible without external input, there is
potential in evaluating solutions in other cases.  We describe three
challenges in this area:

\emparagraph{1. Identifying the causes of policy change:} Identifying and
the causes of change in the security policy is a precondition for
understanding what can and cannot be
addressed with machine learning. Lessons from prior work for file access
policy stability may apply here~\cite{sg09}.

\emparagraph{2. Identifying the time of policy change:} Identifying when a
policy change happens is hard without any input from the user. One
approach to address this challenge is to encourage users to report
policy changes, by taking lessons from persuasive
technologies~\cite{cml09,mc12,pgb+10}.

\emparagraph{3. Identifying the example(s) to change:} The learner may be
able to use existing information (e.g., tag weights, frequency in
examples) to predict which example or tag may be likely to change. Our
intuition is that strategies used for cache replacement (e.g., least
recently used or LRU~\cite{sj94}) may apply, at least as a
starting point.

Finally, active learning may also be used to suggest new examples to the
user, which is not the focus of this paper, and lies in the broader
scope for future work.
%Instead, the focus of \pbe is on predicting the user's policy decisions
%for new scenarios.
%Generating new examples lies in the broader scope for future work.



==> old/intro.tex <==
\section{Introduction}
\label{sec:intro}

In the era of pervasive computing, security of user data and resources
is of paramount importance.  Increasingly complex systems such as IoT
platforms (e.g., IFTTT~\cite{tt10} and SmartThings~\cite{smartthings}), smartphone platforms (e.g., Android and
iOS), and even traditional commodity platforms are being leveraged for
processing user data. However, our knowledge of policy
specification has not kept pace with the rise of complex systems that
are increasingly relying on the user to specify the security policy.

Further, user data has become increasingly user-specific.  Users no
longer directly deal with generic files, but create specific data
objects such as notes, whiteboard snapshots, and selfies. This data is
abstract, i.e., its importance and properties are subjective.  System
designers or application developers cannot specify a security policy
for abstract user data. The situation is even critical for novel
security systems that provide strong data security guarantees for
user data (e.g., decentralized information flow control (DIFC)
systems for Android~\cite{ne13,jaf+13,xw15,naej16},
Chromium~\cite{bcj+15}). Such systems are impractical to deploy unless
users specify security policies; and users are bad at specifying
security policies~\cite{shc+09,mr05} without assistance.

This paper raises the simple but important question of policy
specification: how to teach the system {\em what} the user wants to
protect, and {\em how} the user wants to protect it?  Consider the
following example: a smartphone user wants to synchronize all personal
notes with her cloud account, except notes labeled as medical data.
Since we are dealing with user-specific data-use scenarios, we can
justifiably expect the user to provide some input to the system.
However, expecting the user to enumerate every possible scenario
involving medical data is impractical. The policy must be predicted.

% Making policies great again.

We propose the approach of specifying Policy by Example (\pbe) for
user-specific data. \pbe is inspired by the successful use of
programming by example (PBE) for program synthesis. Specifically, we
emulate the approach of Gulwani~\cite{gul11}, where the user specifies
examples consisting of the input and output, and the system learns a
program that can predict the output for unknown (but similar) inputs.
Similarly, in \pbe, the user specifies policy examples, in terms of the
data-use scenario (i.e., the input) and the policy decision (i.e., the
output).  The system uses the policy examples to predict policy
decisions for new scenarios. By requiring only relevant examples, and
not complete policy specification, \pbe makes policy specification
tractable.

Predicting security policies for abstract, user-specific data with
unknown properties is hard, as the learner cannot make any assumptions
about the input data points. In contrast,
prior work on predicting privacy policies for well-known private
data~\cite{khsc08,cms11} can make assumptions that aid prediction; e.g.,
Cranshaw et al.~\cite{cms11} take advantage of probabilistic models to
learn location privacy policies knowing that location and time are
continuous variables. \pbe cannot make any such assumptions, which puts
us at a significant disadvantage.  However, this disadvantage drove us
to embrace a simpler approach that does not demand specific properties
from data.

We chose a variant of the {\it $k$ nearest neighbor (kNN)}
classifier~\cite{mur12} for predicting policies. Our key requirements
were that the algorithm must be {\sf (1)} non-parametric, i.e.,
independent of probabilistic models that rely on fixed set of
parameters, and {\sf (2)} easy to explain, i.e., for the user to
understand how the policy was inferred. Recall that a policy example is
composed of a scenario and the policy decision for that scenario. For
predicting the policy decision for a new scenario, our algorithm
performs a nearest neighbor search for finding similar scenarios from
the user's policy examples, and predicts the policy decision of the
majority. 

An important challenge in applying kNN is calculating the distance
between data points. For calculating the distance between policy
examples, we treat scenarios as Boolean functions, and propose a novel
distance metric for Boolean functions.  Further, we recognize that some
policies may be more important to the user than others, and extend our
metric to support weights.  Note that existing distance metrics (e.g.,
{\em jaccard} distance) would require significant re-engineering to
incorporate weights, which motivates our development of a new metric.

\pbe recognizes that policy specification by users in any form is error
prone.  A key contribution is our use of active learning for enabling
the user to correct policy decisions. We draw inspiration from the work
of Gulwani~\cite{gul11}, which detects noise in the user's examples, and
prompts the user for new outputs for problematic examples. Similarly,
\pbe uses noise in the user's policy examples as an indication of error
in policy decisions, and engage the user in correcting errors. 
%We define noise for policy examples in terms of invariants on the
%nearest neighbor graph.

We evaluate the feasibility of \pbe with a study of expert
users. Our study involves 8 participants, and 5 target security
policies. As a result, we solve 40 independent policy specification
problems. Our participants generate 246 policy scenarios in total (30 on
average), and assign policy decisions for 5 policies, resulting in a
total of 1,230 policy examples across participants. We perform two
experiments with this data.  First, we compare the errors in policy
decisions found using a manual review and a \pbe-assisted interactive
review of policy examples. Then, we test \pbe's prediction for randomly
generated scenarios with unknown policy decisions. 

\pbe demonstrates a prediction accuracy of over 76\% across all
participants, and fares better than our assumed baseline of a random
coin flip, and a naive approach.  A significant finding is that our
interactive review approach (i.e., using active learning) helps
participants find {\em five times} as many errors as their manual
reviews.

Our evaluation characterizes the feasibility, i.e., the effectiveness of
PyBE in terms of both prediction accuracy and error identification, but
does not speak to the general usability of PyBE.  While 8 participants
may seem small for a human study, the evaluation is able to answer
important questions through the analysis of user-generated tags and
policy examples (i.e., 1,230 user generated examples). The research
questions answered in the evaluation operate at the level of policy
examples, making the data set sufficiently large for evaluating
feasibility.

\begin{comment}
\pbe demonstrates a prediction accuracy of over 76\% across all users.
More importantly, \pbe fares better on average than our assumed baseline
of a random coin flip, and a naive approach of predicting the majority
decision from the training data.  A significant finding is that our
interactive review approach (i.e., using active learning) helps
participants find {\em five times} as many errors as their manual
reviews.
\end{comment}

The contributions of this paper are as follows:

\begin{itemize}
  \item We introduce the Policy by Example (\pbe) paradigm for
    predicting user-specific security policies. Our approach takes
    labeled policy scenarios from the user, and predicts labels (i.e.,
    decisions) for new policy scenarios, thereby making policy
    specification a tractable problem. 
    %We propose a novel distance metric to apply kNN to policy examples,
    %and extend it to support weights.
  \item We use an interactive approach to assist users in finding
    incorrect policy decisions in their examples. We empirically
    demonstrate its effectiveness over manual policy
    reviews.  
  \item We perform a feasibility study with expert users, and
    demonstrate 76\% average prediction accuracy. \pbe performs better
    than both a baseline as well as a naive approach.  
\end{itemize}

This paper is the first step in our vision of a policy assistant for
user data. With \pbe, we provide an approach for predicting security
policies for user-specific data, and demonstrate its technical
feasibility. Further, we analyze our incorrect predictions, and describe
the lessons we learned in the process.  Finally, we describe challenges
(e.g., usability for non-experts, modeling policy change) and future
research directions in this promising new area.

The remainder of this paper proceeds as follows:
Section~\ref{sec:relwork} describes related work.
Section~\ref{sec:motivation} motivates and defines the problem.
%Section~\ref{sec:background} provides the background.
Section~\ref{sec:pbe} provides an overview of our approach.
Section~\ref{sec:algorithm} describes the \pbes algorithm.
Section~\ref{sec:eval} describes the evaluation of \pbe, and
Section~\ref{sec:results} discusses results.
Section~\ref{sec:analysis_of_results} describes our analysis of results,
and Section~\ref{sec:lessons} describes the lessons learned.
Section~\ref{sec:future} details directions and challenges for future
research.  Section~\ref{sec:discussion} discusses threats to validity.
Section~\ref{sec:conc} provides concluding remarks.


==> old/intro_1.tex <==
\section{Introduction}
\label{sec:intro}

In the era of pervasive computing, security of user data and resources
is of paramount importance.  Increasingly complex systems such as IoT
platforms (e.g., IFTTT~\cite{tt10} and SmartThings~\cite{smartthings}), smartphone platforms (e.g., Android and
iOS), and even traditional commodity platforms are being leveraged for
processing user data. However, our knowledge of policy
specification has not kept pace with the rise of complex systems that
are increasingly relying on the user to specify the security policy.

Further, user data has become increasingly user-specific.  Users no
longer directly deal with generic files, but create specific data
objects such as notes, whiteboard snapshots, and selfies. This data is
abstract, i.e., its importance and properties are subjective.  System
designers or application developers cannot specify a security policy
for abstract user data. The situation is even critical for novel
security systems that provide strong data security guarantees for
user data (e.g., decentralized information flow control (DIFC)
systems for Android~\cite{ne13,jaf+13,xw15,naej16},
Chromium~\cite{bcj+15}). Such systems are impractical to deploy unless
users specify security policies; and users are bad at specifying
security policies~\cite{shc+09,mr05} without assistance.

This paper raises the simple but important question of policy
specification: how to teach the system {\em what} the user wants to
protect, and {\em how} the user wants to protect it?  Consider the
following example: a smartphone user wants to synchronize all personal
notes with her cloud account, except notes labeled as medical data.
Since we are dealing with user-specific data-use scenarios, we can
justifiably expect the user to provide some input to the system.
However, expecting the user to enumerate every possible scenario
involving medical data is impractical. The policy must be predicted.

% Making policies great again.

We propose the approach of specifying Policy by Example (\pbe) for
user-specific data. \pbe is inspired by the successful use of
programming by example (PBE) for program synthesis. Specifically, we
emulate the approach of Gulwani~\cite{gul11}, where the user specifies
examples consisting of the input and output, and the system learns a
program that can predict the output for unknown (but similar) inputs.
Similarly, in \pbe, the user specifies policy examples, in terms of the
data-use scenario (i.e., the input) and the policy decision (i.e., the
output).  The system uses the policy examples to predict policy
decisions for new scenarios. By requiring only relevant examples, and
not complete policy specification, \pbe makes policy specification
tractable.

Predicting security policies for abstract, user-specific data with
unknown properties is hard, as the learner cannot make any assumptions
about the input data points. In contrast,
prior work on predicting privacy policies for well-known private
data~\cite{khsc08,cms11} can make assumptions that aid prediction; e.g.,
Cranshaw et al.~\cite{cms11} take advantage of probabilistic models to
learn location privacy policies knowing that location and time are
continuous variables. \pbe cannot make any such assumptions, which puts
us at a significant disadvantage.  However, this disadvantage drove us
to embrace a simpler approach that does not demand specific properties
from data.

We chose a variant of the {\it $k$ nearest neighbor (kNN)}
classifier~\cite{mur12} for predicting policies. Our key requirements
were that the algorithm must be {\sf (1)} non-parametric, i.e.,
independent of models that rely on fixed set of parameters, and {\sf
(2)} easy to explain, i.e., for the user to understand how the policy
was inferred. Recall that a policy example is composed of a scenario and
the policy decision for that scenario. For predicting the policy
decision for a new scenario, our algorithm performs a nearest neighbor
search for finding similar scenarios from the user's examples,
and predicts the policy decision of the majority. 
To calculate distance between scenarios, we treat scenarios as Boolean
functions, and propose a novel distance metric for Boolean functions. As
some policies may be relatively more important to the user, we extend
our metric to support weights. Note that existing distance metrics
(e.g., {\em jaccard} distance) may require significant re-engineering to
incorporate weights, which motivates our development of a new metric.

\begin{comment}
An important challenge in applying kNN is calculating the distance
between data points. For calculating the distance between policy
examples, we treat scenarios as Boolean functions, and propose a novel
distance metric for Boolean functions.  Further, we recognize that some
policies may be more important to the user than others, and extend our
metric to support weights.  Note that existing distance metrics (e.g.,
{\em jaccard} distance) would require significant re-engineering to
incorporate weights, which motivates our development of a new metric.
\end{comment}

\pbe recognizes that policy specification by users in any form is error
prone.  A key contribution is our use of active learning for enabling
the user to correct policy decisions. We draw inspiration from the work
of Gulwani~\cite{gul11}, which detects noise in the user's examples, and
prompts the user for new outputs for problematic examples. Similarly,
\pbe uses noise in the user's policy examples as an indication of error
in policy decisions, and engage the user in correcting errors. 
%We define noise for policy examples in terms of invariants on the
%nearest neighbor graph.

We evaluate the feasibility of \pbe with a study of expert
users. Our study involves 8 participants, and 5 target security
policies. As a result, we solve 40 independent policy specification
problems. Our participants generate 246 policy scenarios in total (30 on
average), and assign policy decisions for 5 policies, resulting in a
total of 1,230 policy examples across participants. We perform two
experiments with this data.  First, we compare the errors in policy
decisions found using a manual review and a \pbe-assisted interactive
review of policy examples. Then, we test \pbe's prediction for randomly
generated scenarios with unknown policy decisions. 

\pbe demonstrates a prediction accuracy of over 76\% across all
participants, and fares better than our assumed baseline of a random
coin flip, and a naive approach.  A significant finding is that our
interactive review approach (i.e., using active learning) helps
participants find {\em five times} as many errors as their manual
reviews.

Our evaluation characterizes the feasibility, i.e., the effectiveness of
PyBE in terms of both prediction accuracy and error identification, but
does not speak to the general usability of PyBE.  While 8 participants
may seem small for a human study, the evaluation is able to answer
important questions through the analysis of user-generated tags and
policy examples (i.e., 1,230 user generated examples). The research
questions answered in the evaluation operate at the level of policy
examples, making the data set sufficiently large for evaluating
feasibility.

\begin{comment}
\pbe demonstrates a prediction accuracy of over 76\% across all users.
More importantly, \pbe fares better on average than our assumed baseline
of a random coin flip, and a naive approach of predicting the majority
decision from the training data.  A significant finding is that our
interactive review approach (i.e., using active learning) helps
participants find {\em five times} as many errors as their manual
reviews.
\end{comment}

The contributions of this paper are as follows:

\begin{itemize}
  \item We introduce the Policy by Example (\pbe) paradigm for
    predicting user-specific security policies. Our approach takes
    labeled policy scenarios from the user, and predicts labels (i.e.,
    decisions) for new policy scenarios, thereby making policy
    specification a tractable problem. 
    %We propose a novel distance metric to apply kNN to policy examples,
    %and extend it to support weights.
  \item We use an interactive approach to assist users in finding
    incorrect policy decisions in their examples. We empirically
    demonstrate its effectiveness over manual policy
    reviews.  
  \item We perform a feasibility study with expert users, and
    demonstrate 76\% average prediction accuracy. \pbe performs better
    than both a baseline as well as a naive approach.  
\end{itemize}

This paper is the first step in our vision of a policy assistant for
user data. With \pbe, we provide an approach for predicting security
policies for user-specific data, and demonstrate its technical
feasibility. Further, we analyze our incorrect predictions, and describe
the lessons we learned in the process.  Finally, we describe challenges
(e.g., usability for non-experts, modeling policy change) and future
research directions in this promising new area.

\begin{comment}
The remainder of this paper proceeds as follows:
Section~\ref{sec:relwork} describes related work.
Section~\ref{sec:motivation} motivates and defines the problem.
%Section~\ref{sec:background} provides the background.
Section~\ref{sec:pbe} provides an overview of our approach.
Section~\ref{sec:algorithm} describes the \pbes algorithm.
Section~\ref{sec:eval} describes the evaluation of \pbe, and
Section~\ref{sec:results} discusses results.
Section~\ref{sec:analysis_of_results} describes our analysis of results,
and Section~\ref{sec:lessons} describes the lessons learned.
Section~\ref{sec:future} details directions and challenges for future
research.  Section~\ref{sec:discussion} discusses threats to validity.
Section~\ref{sec:conc} provides concluding remarks.
\end{comment}


==> old/lessons.tex <==
\section{Lessons}
\label{sec:lessons}

%As seen in Section~\ref{sec:analysis_of_results}, many incorrect
%predictions of \pbe can be resolved by making a few simple but
%significant improvements (e.g., setting weights according to security
%preferences) to the application of \pbe. 
In this section, we describe lessons we learned from our study with
expert users.  These lessons address aspects of correctly using \pbe in
practice, and also motivate problems for future work.

\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=3in]{figs/equalizer}
    \caption{Setting weights using a graphic equalizer, by asking the
    question ``How frequently would you export this data to the Work Cloud?''} 
    \label{fig:policy-equalizer}
\end{figure} 
\end{comment}


\lessonparagraph{Lesson 1: Weight assignment should reflect security,
and not just general privacy preferences.} As seen in our study, the
policy (target) may be semantically related to the tags (e.g., work data is more
confidential with respect to the {\em PersonalCloud}). A generic weight
assignment for multiple policies is bound to be inaccurate.  
%Thus,
%weights should be declared independently for each policy, to reflect the
%policy-specific security preferences of the user.  The usability
%challenge of doing so in a way that is not burdensome to the user is
%discussed in Section~\ref{sec:future}.

\lessonparagraph{Lesson 2: Addressing the problem of ``potential''
change in the user's policy is imperative.} As we discovered in our
study (described in Section~\ref{sec:analysis_of_results}), the user may
change some or all of their security policy goals, but never inform the
policy assistant.  Thus, adapting to potential change in the user's
policy is a major requirement, and a challenge for future work.
%Even if we exempt sudden changes in the user's circumstances (e.g.,
%change in employment), can we predict a potential change in the user's
%policy, while only looking at the current state of the policy examples?
%Our intuition is that \pbe's active learning methodology may be extended
%to address this challenge, as we describe in Section~\ref{sec:future}.

\lessonparagraph{Lesson 3: There might be more than one notion of
``importance'' depending on the security goals.} During our study, we
observed instances where participants wanted to assign more importance
to non-confidential data.  As our study was conducted with strong
security requirements in mind, we did not account for such cases.
Incorporating such a requirement into \pbe is feasible, although the
numeric limits on weights of the confidential and non-confidential tags
must reflect the security goals; i.e., if security is a priority, then the
maximum possible weight for the most confidential tag should be higher
than that for the most non-confidential tag. If usability is a priority,
then the most non-confidential tag may a receive higher weight. 

\lessonparagraph{Lesson 4: Tag semantics should be carefully considered
while applying \pbes.} A small number of our incorrect predictions were
due to ambiguity associated with specific tags as described in
Section~\ref{sec:analysis_of_results}. That is, tags were defined such
that \{{\tt Work,Photo}\} could mean photo created at work, as well as
some work data and an unrelated photo combined. One simple solution
could be to use a separate representation to denote data created at a
particular location or time. For example, a photo created at work may
have the tag {\tt WorkPhoto}, while a derived data object containing
unidentified work data and a photo from an unknown location forms \{{\tt
Work,Photo}\}. This solution and its implications will be explored in
the future.


%lessons that demonstrate the caution that must be taken
%while using \pbe, as well as motivate work in unexplored areas.


==> old/motivation.tex <==
\section{Motivation and Problem}
\label{sec:motivation}

User data and data-use scenarios are user-specific. External observers
such as system designers or application developers cannot specify the
user's security policy without knowing the user's context of data
use~\cite{nis04,bdmn06}. Moreover, this constraint is not limited to
user-owned data; prior work demonstrates that even the security
preferences for enterprise data vary with users and personal data-use
contexts~\cite{gs10}.

Our motivating example demonstrates how two users may differ in terms of
the relevance of data-use scenarios as well as security preferences for
the same scenarios. We then describe the problem addressed by this
paper.

\subsection{Motivating Example}
Alice and Bob are two smartphone users, who use a fictional note-taking
application {\em Notes} (similar to Google Keep) on their smartphones to
collect and organize information. Consider two data-use
scenarios for Alice and Bob, as follows:

%We start out by describing two scenarios involving data secrecy
%policies. 
\subsubsection*{Scenario 1}
%Scenarios involving secret data varies from user to user.  For
%instance,
Alice consolidates expenses by scanning paper receipts into the {\em
Notes} application, which then syncs the receipts with Alice's cloud
provider (such as Google Drive). Alice trusts the cloud with most
information, with the exception of medical data.  Hence, when Alice
scans a receipt from the hospital, she still wants to store it locally
with {\em Notes}, but does not want it exported to the cloud.

Similarly, Bob uses {\em Notes} to aggregate all documents, i.e., data
created or scanned using the smartphone and saved as documents using {\em
Notes}.  Bob's notes are backed up to Bob's enterprise cloud by default.
Bob wants to backup all notes, except personal documents
created after work hours.

\subsubsection*{Scenario 2} Alice and Bob meet at a conference and
exchange business cards. As Alice is self-employed, she feels confident
in backing up all business cards acquired after work hours to her
enterprise cloud.  Bob, on the other hand, does not want to disclose
networking opportunities to his company. Hence, Bob does not want
business cards collected after work hours to be backed up to the
enterprise cloud.

\myparagraph{Observations} We make two observations from the scenarios:
\begin{enumerate}[label=\textbf{O\arabic*},ref=\textbf{O\arabic*}]
  \setlength{\itemsep}{0pt} 
%
\item \label{lesson:what} {\em User data and data-use scenarios are
  diverse.} As seen in Scenario 1, different users may have different
  answers for what scenarios/conditions are applicable to them. Alice
  cares about medical receipts, which may not be relevant to Bob, who in
  turn cares about personal documents. 
%
\item \label{lesson:how}  {\em Security preferences for user data stem
  from the user's personal circumstances}. Even if two users face the
  same scenario, they may not make the same decision on how they want to
  protect their data. In Scenario 2, Alice and Bob both collect business
  cards after work hours, but make different choices based on their
  respective employment situations.
\end{enumerate}

%% The problem
\subsection{The Problem} 
In this paper, we focus on the problem of specifying user-specific
security policies.  The nature of the problem dictates that the policy
specification must receive input from the user. However, it is
impractical to expect the user to specify the policy for every scenario
in an exponential space.  Hence, this paper addresses the problem of
predicting the security policy for new data-use scenarios, based on the
scenarios previously described by the user. 

\begin{comment}
Consider Bob's policy from the motivating example. On his own, Bob may
be able to specify a couple of policy scenarios, e.g., {\sf (1)} {\em
deny} export of business cards collected after work hours, and {\sf (2)}
{\em allow} export of photos.  Now consider a new situation where a
photo clicked after work hours is being exported. What policy should we
apply to this new scenario?  One may argue that the mechanism should
allow access, as one of Bob's policy rules states that photos can be
exported. On the other hand, it is also possible that Bob intended to
deny the export of all data collected after hours, but failed to
indicate as such specifically for photos.  Our approach predicts the
security policy when the complete policy specification may not be
available. 
\end{comment}

\begin{comment}
An immediate challenge in solving this problem is the sample size and
distribution of data available to the learner. The training set is bound
to be small, as the model for user-specific policies may only use data
provide by the specific user.  Further, the user may not adhere to a
specific probability distribution.  Hence, traditional classification
algorithms that require large datasets or a known probability
distribution to provide meaningful results may not be suitable to solve
the problem.
\end{comment}


==> old/overview.tex <==
\section{Policy by Example (\pbe)} 
\label{sec:pbe}

%This paper proposes Policy by Example (\pbe), an approach for specifying
%policies for user-specific resources.  \pbe focuses on predicting the
%user's policy specification, and is the first step in realizing our
%vision of a policy assistant for creating and managing security policies
%for user resources. 

\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=2.8in]{figs/overview}
    \caption{Overview of the \pbe approach.}
   \label{fig:overview}
   \vspace{-1em}
\end{figure}
\end{comment}

\begin{figure}[t]
  \centering
  \subfloat[][The user specifies examples. \pbe suggests
  error-correction.]{\includegraphics[width=1.2in]{figs/overview_a}\label{fig:overview_a}}\qquad
  \subfloat[][\pbe predicts policy decisions for new
  scenarios.]{\includegraphics[width=1.4in]{figs/overview_b}\label{fig:overview_b}}
  \vspace{-0.8em}
  \caption{An overview of the \pbe approach.}
  \label{fig:overview}
  \vspace{-1.5em}
\end{figure}

\pbe is inspired by recent work on Programming by Examples~\cite{gul11},
which learns a program from input-output examples. As shown in
Figure~\ref{fig:overview_a}, the user provides policy examples (i.e.,
data-use scenarios and policy decisions), and \pbe interactively
suggests corrections to the user's policy decisions.  \pbe then predicts
policy decisions for new scenarios as shown in
Figure~\ref{fig:overview_b}.

This section provides the intuition behind our approach. We describe
\pbe formally in Section~\ref{sec:algorithm}.  We start by describing
the structure of a policy example.
%The
%user specifies a set of policy examples and weights (described later) as
%input for \pbe, and \pbe predicts the policy decisions for new examples.

\subsection{The Policy Example} 
\label{sec:policy-example}
%The user must be able to express complex scenarios composed of multiple
%conditions or data types in a policy example.  
A policy example is composed of a {\em scenario}, and a {\em policy
decision} (i.e., {\sf allow}/1 or {\sf deny}/0) for that scenario. A
scenario is as a set of {\em tags}, where each tag denotes the resource
to be protected (e.g., business card) or a condition that influences the
policy (e.g., created after work hours). Using a set of tags enables
users to describe complex scenarios composed multiple conditions or data
objects. Our use of tags is motivated by prior work that
demonstrates that users can effectively re-purpose organizational tags
to express access control policies~\cite{klms+12}. 

In addition to the user-customizable policy example, we also define a
fixed policy {\em target} which represents the action controlled
by the policy; e.g., exporting data to the enterprise cloud, i.e.,
the {\em WorkCloud} policy target. Policy specification
is performed separately for each policy target, i.e., independent of
other targets. Thus, each target represents a separate
high-level policy that must be specified (e.g., the user's {\em
WorkCloud} policy).  The policy targets used in this paper are motivated
by prior work on restricting the network export of secret data~\cite{sym+14,bcj+15,naej16}.

% Bobs example.
\begin{table}[t]
\footnotesize
\centering
\caption{Bob's examples for the {\em WorkCloud} policy.}
\vspace{-0.5em}
\label{tbl:bob-policy}
\begin{tabular}{l|c|c}
  \Xhline{2\arrayrulewidth}
  {\bf No.} & {\bf Scenario}             & {\bf Policy Decision}\\
  \Xhline{2\arrayrulewidth}
  1 & \{Home, Photo\}   & deny  \\  
  2 & \{Work, Photo\}   & allow  \\  
%  3 & \{Photo\}   & DENY  \\  
  3 & \{Document\} & allow \\
  %4 & Home $\wedge$ Document & DENY \\
  \Xhline{2\arrayrulewidth}
    \end{tabular} 
    \vspace{-1.5em}
\end{table} 

Table~\ref{tbl:bob-policy} shows Bob's policy examples for the {\em
WorkCloud} policy target. We describe each example, along with Bob's
security requirement associated with it.
%Bob provides this set of examples as input to \pbe. 
%Each example is associated with one or more of Bob's security
%requirements.  
First, Bob considers data created at home to be personal, so Bob's
photos created at home must never be exported to the enterprise cloud.
Thus, Bob denies export for example~1, i.e, \{{\tt Home,Photos}\}.
Second, photos taken at work may be exported to the enterprise cloud.
Hence, Bob allows export for example~2, i.e., \{{\tt Work,Photos}\}.
Third, Bob does not (currently) imagine a situation where he would deny
export for documents.  Hence, Bob allows export for example~3, i.e.,
\{{\tt Document}\}.  We now use Bob's examples to informally describe
\pbe. Our algorithm is formally described in Section~\ref{sec:algorithm}.

\subsection{Our Approach}
\label{sec:overview}

As described previously, \pbe uses a variation of the kNN algorithm for
predicting policies. That is, Bob provides \pbe with a set of policy
examples (i.e., scenarios labeled with policy decisions). When faced
with a new scenario with an unknown policy decision, we perform a
nearest neighbor search of Bob's examples. That is, we search Bob's
examples for the closest examples, i.e., examples with scenarios closest
to the new scenario, and predict the policy decision of the majority of
the closest examples.  Note that distance between examples is described
in terms of their scenarios (i.e., when we say ``examples are close'',
it means their scenarios are close). 

An approach for predicting security policies should be deterministic if
we want users to understand its outcome (i.e., independent of arbitrary
parameters).  Based on this rationale, we eliminate the need to specify
the parameter $k$. Our variation of kNN considers the {\em closest}
neighbors as all neighbors at the closest distance, instead of k
neighbors at varying distances.

We now demonstrate our approach with a manual walk-through. A manual
walk-through is feasible because the basic process of kNN is intuitive
and its outcome is easy to explain. 
To demonstrate our approach, we predict
policy decisions for the following new scenarios for Bob: \{{\tt Home}\}
and \{{\tt Home,Document}\}, using Bob's initial policy specification
shown in Table~\ref{tbl:bob-policy}.

Consider the first new scenario, \{{\tt Home}\}.  Just by looking at
Bob's specification in Table~\ref{tbl:bob-policy}, the reader may
identify example~1 (i.e., \{{\tt Home,Photo}\}) as closest to the new
scenario, since it is the only example that includes the tag {\tt Home}.
As a result, we predict the policy decision for the new scenario
{\tt \{Home\}} as {\sf deny}, i.e., as the decision of its nearest
neighbor \{{\tt Home,Photo}\}. This decision mirrors Bob's assumption of
data created at home being personal, and not exportable to the
enterprise cloud. \pbe's distance metric described in
Section~\ref{sec:algorithm} uses a similar property for computing
distance between two examples, and comes to the same conclusion. 

Now consider the second new scenario, \{{\tt Home,Document}\}. This
time, there are two examples that seem to be equally close to the new
scenario, i.e., \{{\tt Home,Photo}\} and \{{\tt Document}\}, since they
each
have one tag in common with \{{\tt Home,Document}\}. Since both the
nearest examples have different policy decisions, our simple metric is
insufficient. This is one of the motivations for introducing
weights.  Suppose Bob considers personal data created at home (i.e., the
tag {\tt Home}) to be most confidential. Therefore, Bob assigns {\tt
Home} more ``importance'' (i.e., a higher weight) than any other tag in
terms of its influence on the policy decision.  As a result, the new
scenario \{{\tt Home,Document}\} can be deemed closer to \{{\tt
Home,Photo}\} than \{{\tt Document}\}, as {\tt Home} has a higher weight
and more say in the decision than the other tags, e.g.,
{\tt Document}. Thus, export is denied for \{{\tt Home,Document}\},
which aligns with Bob's preference of data created at home being
personal, and not exportable to the enterprise cloud. 

The purpose of weights is not limited to breaking ties. Suppose Bob
specifies another example \{{\tt Document,Receipt}\} with decision {\sf
allow}. Now consider another new scenario \{{\tt
Document,Receipt,Home}\}. Without any knowledge of weights, it is easy
to see that \{{\tt Document,Receipt}\} would be the example closest to
the new scenario \{{\tt Document,Receipt,Home}\}, resulting in {\sf
allow} being predicted (i.e., there is no tie).  At the same time, we
know that Bob has allocated a higher weight to {\tt Home}, since Bob
considers home data to be confidential and important with respect to the
{\em WorkCloud} target. The weights ensure that \{{\tt
Document,Receipt,Home}\} is closer to \{{\tt Home,Photo}\} instead of
\{{\tt Document,Receipt}\}, and export is denied as per Bob's actual
security preference. Simply stated, weights enable the user to make some
information tags beat others in the distance calculation.  Our weighted
metric described in Section~\ref{sec:weighted-metric} uses a similar
reasoning.

% Bobs example.
\begin{table}[t]
\footnotesize
\centering
\caption{Bob's extended set of examples for the {\em WorkCloud} policy target, with newly added examples in {\bf bold}.}
\vspace{-1em}
\label{tbl:bob-policy-revised}
\begin{tabular}{l|c|c}
  \Xhline{2\arrayrulewidth}
  {\bf No.} & {\bf Scenario}             & {\bf Policy Decision}\\
  \Xhline{2\arrayrulewidth}
  1 & \{Home, Photo\}   & deny  \\  
  2 & \{Work, Photo\}   & allow  \\  
%  3 & \{Photo\}   & DENY  \\  
  3 & \{Document\} & allow \\
  {\bf 4} & \{{\bf Home, Document}\} & {\bf deny} \\
  {\bf 5} & \{{\bf Home, Memo}\} & {\bf allow} \\
  %4 & Home $\wedge$ Document & DENY \\
  \Xhline{2\arrayrulewidth}
    \end{tabular} 
\vspace{-1em}
\end{table} 

An important contribution of \pbe is that it recognizes that policy
specification by users can be error-prone. \pbe uses active learning to
engage the user in finding and correcting potential errors in their
policy decisions.  Our approach is inspired by the work of
Gulwani~\cite{gul11}, which detects noise in the user's input-output
examples, and recommends changes to incorrect outputs.
Similarly, \pbe looks for noise in the user's examples, which may
indicate one or more incorrect policy decisions.  We use our
variant of kNN for this purpose.  Note that the objective of this task
is to engage the user in finding errors in existing examples, and not to
predict policy decisions for new examples.  We explain our approach with
the following extension to Bob's policy:

Suppose Bob adds two additional examples, i.e., \{{\tt Home,Document}\}
with decision {\sf deny}, and \{{\tt Home,Memo}\} with decision {\sf
allow}. We borrow the first example (i.e., for a document created at
home) from the previous discussion on weights. The second example shows
Bob's policy for a memo created at home.  Further, recall that {\tt
Home} has a higher weight, hence examples containing {\tt Home} will be
closer to each other than other examples not containing {\tt Home}.
Bob's complete set of examples is shown in
Table~\ref{tbl:bob-policy-revised}.

We perform a nearest neighbor search for the example \{{\tt Home,
Memo}\}, and identify \{{\tt Home, Photo}\} and \{{\tt Home, Document}\}
as its nearest neighbors. An intuitive way of visualizing this group of
examples is in the form of a graph, such that {\sf (1)} the examples are
vertices, and {\sf (2)} directed edges are drawn from the example for
whom the search was performed to its nearest neighbors.
%\footnote{This is a simplified explanation of the nearest neighbor graph
%to provide intuition; a more formal definition can be found in
%Section~\ref{sec:active-learning}.} 
Figure~\ref{fig:nn-graph-a} shows the graph for \{{\tt Home, Memo}\}.

\begin{figure}[t]
    \centering
    \includegraphics[width=2in]{figs/nn-graph-a}
    \vspace{-0.5em}
    \caption{\{{\tt Home, Memo}\} disagrees with the majority policy decision of its
    nearest neighbors.} 
    \label{fig:nn-graph-a}
    \vspace{-1.5em}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=2in]{figs/nn-graph-c}
    \vspace{-0.5em}
    \caption{
    There is no majority policy decision among the nearest neighbors of \{{\tt
    Home, Photo}\}.
    } 
    \label{fig:nn-graph-c}
    \vspace{-1.5em}
\end{figure}

If we focus on the policy decisions of the vertices in
Figure~\ref{fig:nn-graph-a}, we see that Bob's decision for \{{\tt Home,
Memo}\} (i.e., {\sf allow}) disagrees with the decision for both its
nearest neighbors. This inconsistency or noise indicates one of two
possibilities: {\sf (a)} Bob made a mistake in labeling \{{\tt Home,
Memo}\} with the decision {\sf allow}, or {\sf (b)} Bob wanted to make a
genuine exception for memos. Instead of making a guess, \pbe asks Bob.
That is, we recommend Bob to label \{{\tt Home,Memo}\} as {\sf deny} for
resolving this inconsistency, Bob may accept our recommendation, or
reject it and make an exception. Using such interactive recommendations,
\pbe engages Bob in correcting potential errors. 


Figure~\ref{fig:nn-graph-c} shows the nearest neighbor graph for \{{\tt
Home,Photo}\}, and illustrates another type of inconsistency. In this
case, there is no majority consensus among the neighbors of \{{\tt
Home,Photo}\}. A similar situation exists in the graph for \{{\tt
Home,Document}\}, which we do not show due to space constraints. If we
look at the two graphs in Figure~\ref{fig:nn-graph-a} and
Figure~\ref{fig:nn-graph-c}, we realize that changing the policy
decision of \{{\tt Home,Memo}\} removes both the inconsistencies. Thus,
\pbe capitalizes on the possibility that a few examples may cause the
most noise, and recommends the user to change their labels.  In our
algorithm described in Section~\ref{sec:active-learning}, we describe
graph invariants to identify noise, and a greedy algorithm to find the
optimal change. Section~\ref{sec:results} demonstrates that our
interactive approach finds {\em five times} as many errors as manual
reviews by users.

Note that we do not claim to detect all errors, as the users' examples
may be completely consistent, but may still have errors. Instead, we
recommend a best effort approach for engaging the user in detecting
potential errors. 
%More optimal solutions may be incorporated into \pbe in the future.
\begin{comment}
In fact, similar graphs can be drawn for the \{{\tt Home, Photo}\} and \{{\tt
Home, Document}\}, as shown in Figure~\ref{fig:nn-graph-b} and
Figure~\ref{fig:nn-graph-c} respectively.
  \centering
  \subfloat[][\{{\tt Home, Memo}\} disagrees with its majority neighbors]{\includegraphics[width=1.5in]{figs/nn-graph-a}\label{fig:nn-graph-a}}\\
  \subfloat[][There is no majority in the neighbors of \{{\tt Home, Photo}\}]{\includegraphics[width=1.5in]{figs/nn-graph-b}\label{fig:nn-graph-b}}\quad
  \subfloat[][There is no majority in the neighbors of \{{\tt Home, Document}\}]{\includegraphics[width=1.5in]{figs/nn-graph-c}\label{fig:nn-graph-c}}
  \caption{Nearest neighbor graph for the example scenarios \{{\tt Home,
Memo}\}, \{{\tt Home, Photo}\} and \{{\tt Home, Document}\}. The vertices are
examples, and edges are drawn from the example for whom the nearest neighbor
search was performed, to its nearest neighbors. Vertices are labeled with their policy decisions.}
\label{fig:nn-graph}
\end{figure}
\end{comment}



==> old/relwork.tex <==
\section{Related Work}
\label{sec:relwork}

The notion of Policy by Example (\pbe) is directly influenced by recent
work in the domain of Programming by Example (PBE).\footnote{Also
sometimes called Programming by Demonstration} The objective of PBE is
simple: if the user knows the steps in performing a task, the user
should not have to write a program; instead, the computer should learn
from the user's actions on an example, and generalize a corresponding
program~\cite{ch93,lie01}. However, the user may not always be able to
express the reasoning, or the intermediate steps, involved in creating a
program (i.e., converting an input to the desired output).
Gulwani~\cite{gul11} makes PBE a feasible approach for such programming
tasks, where the user may only have the input and the corresponding
output for each example, by using only input-output examples to
synthesize a program that predicts outputs for unseen inputs (e.g.,
creating Excel macros). \pbe follows a similar intuition, and predicts
the policy decisions using only input-output
examples provided by the users, in the form of policy scenarios (i.e.,
the input) and decisions (i.e., the outputs).

However, \pbe does not generalize the program, as is often done in PBE.
That is, while the proposed paradigm is conceptually similar to PBE, the
process used to predict policies borrows from another well-established
domain, that of case-based reasoning~\cite{kol93}. In case-based
reasoning, the outcome of a test case is predicted by directly looking
at the outcomes of previously observed cases (e.g., legal reasoning). In
a way, case-based reasoning mimics a human expert's reasoning. \pbe's
logic of predicting the decision for a test scenario based on the
decisions of ``similar'' previously specified scenarios is a form of
case-based reasoning, and the reason we use this approach is the
uncertainty involved in predicting policies for abstract data.

Case-based reasoning provides a way to deal with uncertainty.  Prior
approaches for predicting user-specific privacy policies for well-known
private data (e.g., Location data) use inductive learning, which
requires the learner to choose a direction for generalization, generally
based on some known properties of the data points~\cite{khsc08,cms11}.
For example,  

However,
case-based reasoning provides a way to deal with uncertainty, i.e., for
scenarios such as ours where the properties of the input data points
(i.e., abstract user data) are unknown.
That is, the approach
does not create a generalization apriori, instead preferring to 

\begin{comment}
In PBE, the system records the repetitive interactions between the user
and a user interface, and generalizes a program to represent the set of
user actions~\cite{,lie01}. PBE teaches the computer a program, i.e.,
new behavior expected by the user, through the demonstration of the
user's actions on an example. However, providing intermediate steps in a
program may require expert knowledge. Gulwani~\cite{gul11} makes PBE a
feasible approach for programming tasks where the user may only have the
input and the corresponding output for each example (e.g., creating
Excel macros). \pbe follows the same intuition, and predicts the output
of a program (i.e., policy decisions) using only input-output examples
provided by the users, in the form of policy scenarios (i.e., the input)
and decisions (i.e., the outputs).
\end{comment}

In this section, we describe prior work on automatic customization of
privacy policies. Additionally, we discuss the complementary areas of
languages for expressing security policies, enforcement of security
policies, and the usability of policy interfaces.

\subsection{Automatic customization of privacy policies}

%% Firewalls, SELinux, for developers or system data. Not user-specific,
% but drawing from the policy goals. Similarly, DIFC and access control
% policy instrumentation based on the developer's policy goals. Policy
% specification for the user's personal resources may need to acquire
% the user's input.

The proposals for user-controllable learning of security and privacy
policies~\cite{khsc08,cms11} are closely related to our vision of a
security policy assistant. Simply stated, user-controllable learning
allows the user to actively participate in policy customization, which
is also an objective of \pbe. However, our objective is to specify
policies for abstract user-specific data objects (e.g., Bob's office
documents), while prior work on user-controllable learning specifies
policies for well-known private data or security preferences (e.g.,
Location data).  As a result, \pbe cannot make any assumptions about the
properties of the data to be protected while making predictions. On the
contrary, user-controllable learning leverages well-known properties of
data for predicting policies. For instance, Cranshaw et al.~\cite{cms11}
use a probabilistic model for prediction of location privacy policies,
with the underlying assumption that a large number of data points would
be available since location and time are continuous variables.  \pbe's
approach of treating data or conditions as abstract objects is necessary
for policy specification for user-specific data.

Machine learning has frequently been used to tag user content for access
control~\cite{vscy09,sslw11,slb13,bbzl15,slsw15}. For instance, Sinha et
al.~\cite{slb13}  predict privacy preferences for Facebook users by
classifying Facebook posts into various Facebook sharing policies.  \pbe
supports finer-grained policies, where different classes of content
(i.e., tags) do not directly map to security policy decisions, but can
instead be combined by the user into different policy scenarios.
However, such prior approaches are complementary, as their content
recognition techniques can be leveraged to automatically tag content for
\pbe.  Applications such as {\em Google Photos} use similar methods to
tag content~\cite{google-photos}, and may also be used for \pbe.  
%Further,
%prior work also shows that users can effectively leverage organizational
%tags for specifying security policies~\cite{klms+12}.

% Approaches that use ML to predict the policy decision from data. E.g.,
% predicting the sharing preference (i.e., share with Friends) on
% Facebook for posts containing images, test and URLs.
%% Some approaches for user-specific policy customization 
Prior work in configuring mobile privacy settings states that even if a
one-size-fits-all configuration is infeasible, a small set of privacy
profiles may still be helpful~\cite{lls14,llsh14}. For example, Liu et
al. study the configuration of 12 Android permissions across 4.8 million
users, and cluster the permission settings into a small number of
privacy profiles that apply to large populations~\cite{lls14}. The
approach works for Android permissions as every user configures the {\em same}
Android permissions, although differently. However, user data is
abstract and user-specific, and so is its security value to the user.
Hence \pbe's user-specific approach may be more appropriate for user
data.


Finally, Fang and LeFevre propose a ``privacy wizard'' for setting
social network policies~\cite{fl10}. The approach uses active learning
to specify data sharing policies with respect to the user's friends. 
%The
%privacy wizard uses uncertainty sampling, i.e., it asks the user to
%label the policy for the friends it is most uncertain about at every
%iteration, and learns the policy for all friends over time. 
%In a way, the use of friends by Fang
%and LeFevre is similar to that of policy examples in \pbes, where the
%features of friends are similar to tags used to construct examples. One
%noticeable difference is that the approach deals with a small number of
%features (i.e., 1-5), while the average number of tags used in the
%security policies of our users is 14 (as described in
%Section~\ref{sec:results}. 
A significant difference is that the active learning approach used by
the privacy wizard assumes independence among attributes of data points
(i.e., friends). A similar assumption may not be appropriate for the
data involved in user data scenarios. That is, the policy decision for a
scenario formed by combining tags may be a property of all the tags
combined.  Therefore, our kNN-based approach is more appropriate, as it
does not assume attribute independence.


\subsection{Languages for expressing security policies}

To protect user data held by applications, prior research has provided
application developers with tools for expressing their security and
access control policies~\cite{ek08,he08,hjr10,sxwx14}.  Efstathopoulos
and Kohler~\cite{ek08} provide a policy description language for
applications, to describe their policy for the Asbestos decentralized
information flow control (DIFC) system~\cite{vek+07}. The policy
expressed by developers is compiled into low-level Asbestos primitives.
Boat~\cite{he08} provides similar support for generating policy for the
Flume DIFC model~\cite{kyb+07}, while Harris et al.~\cite{hjr10}
automatically instrument programs with DIFC policy. Further, Slankas et
al.~\cite{sxwx14} aid the developer by extracting access control rules
from application-specific text artifacts using natural language
processing (NLP). Such prior work provides developers with the means
to compartmentalize the application and implement correct access control
policies within the application. While these measures may indirectly
benefit the user, they do not address the lack of policy specification
from the user's perspective.

\subsection{Enforcement of security policies}
%% IFC? Tagging information and propagating tags
In this paper, we allow the specification of policies using example
scenarios that may involve more than one tag, i.e., may indicate
information derived from multiple sources, or the existence of multiple
conditions. A large body of research in access and information flow
control enforces the propagation of tags to enable labeling of derived
content~\cite{bl76,cfg+87,ml97,vek+07,kyb+07,afb+12,ne13,xw15,bcj+15,naej16}.
For instance, Aquifer~\cite{ne13} and the approach by Jia et
al~\cite{jaf+13} provide policy models for enabling the data secrecy on
Android. Maxoid~\cite{xw15} and Weir~\cite{naej16} extend these prior
works by making enforcement of such guarantees practical on Android.

Further, Bauer et al~\cite{bcj+15} provide a policy and enforcement
model for information flow control on the Chromium Web browser.  Prior
work also motivates and enforces the policies similar to the network
export control policy targets used as examples in this
paper~\cite{naej16, sym+14}.  This paper advances the deployment of
these novel systems by making their policy specification feasible.

\subsection{Usability of policy interfaces}
%In this category, we briefly discuss prior work on obtaining policies
%from the user for user-owned resources, and for usable visualization of
%access control policies.

Johnson et al.~\cite{jkkg10a,jkkg10b} propose an interactive policy
authoring template for usable policy specification, and provide a
GUI-based prototype for generating policy templates. A prototype of \pbe
for a computing device may adopt the ``interactive dropdowns'' provided
in the authoring template to ease the task of specifying initial
examples.

Further, Reeder et al.~\cite{rbc+08} propose ``expandable grids'' to
visualize policy rules. A notable aspect of the work is that expandable
grids enable the user to focus on the integrated effect of multiple
policy rules, rather than having to reason about the interactions
between different rules through manual analysis. Such an approach may be
adapted for visualizing policy examples as well, or even for displaying
the predictions generated by \pbe to the user. 

Finally, access control gadgets (ACGs)~\cite{rkm+12} provide a usable
method for acquiring the user's permission for user-owned resources on
modern operating platforms (e.g., Android, iOS, Windows 8), i.e., by
embedding the resource access permission into the user's natural UI flow
of accessing the resource. In a way, ACGs extend prior work that deals
with involving the user in access control decisions for
files~\cite{se08,sky+06}. ACGs make traditional offline policy
specification obsolete, but only for specific coarse-grained resources.
That is, while ACGs may be feasible for a few coarse-grained security
permissions, designing gadgets for an exponential number of personal
data-use scenarios may not be feasible. 


==> old/relwork_1.tex <==
\vspace{-0.5em}
\section{Related Work}
\label{sec:relwork}
\vspace{-0.5em}

The notion of Policy by Example (\pbe) is inspired by recent work in the
domain of Programming by Example (PBE). The objective of PBE is simple:
if the user knows the steps for performing a task, the user should not
have to write a program; instead, the computer should learn from the
user's actions on an example, and generalize the
program~\cite{ch93,lie01}. However, the user may not always be able to
express the reasoning, or the intermediate steps, involved in creating a
program.  Gulwani~\cite{gul11} makes PBE feasible for such programming
tasks, by using only input-output examples to synthesize a program that
predicts outputs for unseen inputs. \pbe
follows a similar intuition, and predicts policy decisions for new
scenarios using only input-output examples (i.e., policy scenarios and
corresponding decisions).

However, \pbe does not generalize the program before testing, as is
often done in PBE.  That is, while the proposed paradigm is conceptually
similar to PBE, the process used to predict policies borrows from
another well-established domain: case-based reasoning
(CBR)~\cite{kol93}. In CBR, the outcome of a test case is determined by
looking at the outcomes of previously observed cases (e.g.,
legal reasoning using precedents). In a way, CBR mimics a human expert's
reasoning, and performs lazy generalization of domain knowledge at
testing time. CBR has been successfully used in many domains, e.g.,
synthesizing music~\cite{ads98,ad01}, providing decision support in
molecular biology~\cite{jrg+01},  and for solving spatial reasoning
problems~\cite{hol99}. However, to our knowledge, CBR has never been
used for predicting user security policies, and \pbe is novel in its use
of a similarity heuristic (i.e., a form of CBR) for predicting security
policies.

A critical advantage of CBR is that it provides a way to deal with
uncertainty, in contrast with the process of eager learning (e.g., rule
induction). Prior user-controllable methods for predicting privacy
policies for well-known private data (e.g., Location) use eager
learning, which requires making strategic parameter choices for
generalization, often based on some known properties of the training
data~\cite{khsc08,cms11}.  For example, Cranshaw et al.~\cite{cms11} use
a probabilistic model to learn location privacy policies, assuming the
availability of a large number of data points since location is a
continuous variable.  However, \pbe cannot make such assumptions for
user data with uncertain properties (e.g., Bob's scanned documents,
Alice's notes), and uses a form of CBR, which does not require a priori
generalization.

%\pbe's logic of predicting the decision for a test
%scenario based on the decisions of ``similar'' previously specified
%scenarios is a form of case-based reasoning.

\begin{comment}
In PBE, the system records the repetitive interactions between the user
and a user interface, and generalizes a program to represent the set of
user actions~\cite{,lie01}. PBE teaches the computer a program, i.e.,
new behavior expected by the user, through the demonstration of the
user's actions on an example. However, providing intermediate steps in a
program may require expert knowledge. Gulwani~\cite{gul11} makes PBE a
feasible approach for programming tasks where the user may only have the
input and the corresponding output for each example (e.g., creating
Excel macros). \pbe follows the same intuition, and predicts the output
of a program (i.e., policy decisions) using only input-output examples
provided by the users, in the form of policy scenarios (i.e., the input)
and decisions (i.e., the outputs).
\end{comment}


%% Firewalls, SELinux, for developers or system data. Not user-specific,
% but drawing from the policy goals. Similarly, DIFC and access control
% policy instrumentation based on the developer's policy goals. Policy
% specification for the user's personal resources may need to acquire
% the user's input.

Prior work also complements the specification of user-specific policies,
by providing content recognition for tagging
Prior research that performs content recognition for tagging can be
leveraged to automatically tag content for
\pbe~\cite{vscy09,sslw11,slb13,bbzl15,slsw15}. Further, prior work for
generating security profiles through large-scale mining of user
preferences provides baseline protection to users for standard,
well-known, security settings (e.g., Android
permissions)~\cite{lls14,llsh14}. \pbe complements this baseline by
predicting policies for abstract, user-specific data, for which an
analysis across users may be infeasible. 

% Fang and LeFevre also assume domain experties; we should move this to
% the previous category with Cranshaw
%Finally, Fang and LeFevre's ``privacy wizard''~\cite{fl10} for social
%network privacy settings assumes attribute independence for data
%points, which may not be appropriate for policy scenarios in \pbe.


\begin{comment}
Finally, Fang and LeFevre also 
use active learning in their ``privacy wizard'' for social network
privacy settings~\cite{fl10}; however, the wizard assumes independence
among attributes of data points, which may not work for data use
scenarios formed by combining different data or conditional tags. In
contrast, \pbe's kNN-based approach does not assume attribute
independence.

Further, Fang and LeFevre
propose an active learning-based approach to create a ``privacy wizard''
for setting social network policies~\cite{fl10}. A significant
difference is that the active learning approach used by the privacy
wizard assumes independence among attributes of data points (i.e.,
friends), which may not be appropriate for user data scenarios formed by
combining different data or conditional tags. In contrast, \pbe's
kNN-based approach does not assume attribute independence.
\end{comment}

This paper is the first step in our vision of creating a policy
assistant, and demonstrates the feasibility of our approach. However,
prior work has proposed usable ways to specify security policies, which
is relevant with respect to our long-term vision.  For instance, a
prototype of \pbe for a computing device may adopt the ``interactive
dropdowns'' in Johnson et al.'s interactive policy authoring template
for specifying initial examples~\cite{jkkg10a,jkkg10b}. Similarly,
Reeder et al's ``expandable grids'' may be adapted for visualizing
policy examples for the user~\cite{rbc+08}. Recent work on access
control gadgets (ACGs)~\cite{rkm+12} by Roesner et al. provide a usable
way of acquiring the user's policy decision, by embedding access
permissions into the user's natural UI flow of accessing resources.
However, this approach only works for well-known resources controlled by
the OS; designing gadgets for an exponential number of personal data-use
scenarios may not be feasible.

Finally, while \pbe assists the user in specifying policies
for user-specific data, there exists prior work in the general area
of policy specification that helps application or system developers.
Prior work provides application developers with tools for expressing
their security policies~\cite{ek08,he08,hjr10,sxwx14}.  Further, in
contrast with prior work that assists developers in expressing known
policies, Slankas et al. aid the developer by extracting access control
rules from application-specific text artifacts using natural language
processing (NLP)~\cite{sxwx14}.  Similarly, access control logs and
system call traces have previously been used to refine the system's
security policies (e.g., EASEAndroid~\cite{wer+15} and
Polgen~\cite{shr06}).



==> old/results.tex <==
\section{Results}
\label{sec:results}

This section describes the results of our experiments, i.e., \pbe's
accuracy in predicting policy decisions for new scenarios, and its
effectiveness in assisting participants in finding incorrect policy
decisions in their examples.  We start by describing the data collected
during the initial policy specification (i.e., the specification
dataset), and the testing dataset.

%\input{dataset_tbl} 
\myparagraph{Specification dataset} 
%Table~\ref{tbl:dataset} shows the number of unique examples collected
%from our expert participants.  
The 8 participants provided 246 example scenarios in total, with policy
decisions for 5 policy targets, resulting in a total of 1,230 initial
labeled policy examples.  Participants used on average 14 tags to
specify their scenarios, with 40 unique tags (available in
Appendix~\ref{app:tags}) used across participants.

%\input{testing_dataset_tbl} 
\myparagraph{Testing dataset}
%Table~\ref{tbl:testing_dataset} shows the size of the testing dataset
%for each participant.  
We generated a total of 122 random test scenarios across 8 participants,
which when labeled with ground-truth policy decisions by participants
for 5 policies, resulted in 610 test examples. 
%Between 10 to 26 new random test scenarios were generated for each
%participant, based on the number of initial examples they provided.
%Participants provided ground-truth policy decisions for 5 policies for
%each scenario, resulting in a total of 610 test examples.  
A detailed split (per participant) of the testing and training datasets
can be found in Appendix~\ref{app:datasets}.

\subsection{Accuracy of Predictions}
\input{coinflip_tbl}
\input{mostfreq_tbl} 
%%ACCURACY (RQ2, RQ3)
Our algorithm predicted decisions for all of the participants' new
(test) policy examples.\footnote{We performed testing with random
samples instead of cross-validation, as the latter is generally
performed to test ``models'', i.e., for supervised learning.} The actual
prediction time was negligible (i.e., less than 1 second for all the
examples for one participant).  Further, for less than 6\% (36 out of
610) of our test examples we had no majority label (i.e., a tie).
Applying the tie-breaker discussed in Section~\ref{sec:no-majority}
resolved 19 of these ties, while the rest (i.e., 3\% or 17 out of 610)
were denied by default. We now discuss the accuracy of \pbe's
predictions.

On comparing our predicted decisions with ground-truth decisions
provided by participants, we observe that \pbes predicts policy
decisions with
an average accuracy of over 76\% across all participants (\ref{rq:accuracy}).
When analyzing the accuracy, it is important to note that each
participant-policy combination is treated as an independent policy
specification problem, and hence forms a separate test case. We first
define a baseline and naive approach against which we evaluate \pbe's
accuracy. 

\myparagraph{1. The CoinFlip baseline} The {\em CoinFlip} baseline provides
the measure of accuracy of random guessing, with an equal probability of
a 0/1 outcome on each flip. 

\myparagraph{2. The MostFreq naive approach} We define {\em MostFreq} as
an approach that predicts the most frequent or majority policy decision
from the initial examples, for the respective participant-policy
problem.  For example, if a participant generally allows in policy
decisions for a certain policy target, {\em MostFreq} will predict allow
for all new test examples for that participant-policy problem.  The
insight behind {\em MostFreq} is that a naive learner is likely to pick
the majority class, in order to benefit from the consistent trend in the
participant's policy decisions.
%Note that we limited testing to the first 5 policies to limit user
%fatigue. 

Table~\ref{tbl:coinflip_perf} shows the comparison of \pbe's accuracy
with {\em CoinFlip}, for each of the 40 participant-policy cases (i.e.,
8 participants and 5 policy targets). \pbe performs better than {\em
CoinFlip} in all but 3 cases (i.e., 92\% of the time). \pbe's average
accuracy of over 76\% is better than {\em CoinFlip} (50\% accuracy).
Additionally, \pbe performs better than {\em CoinFlip} for all 8
participants, across all policies.
%when we average the accuracy for all policy targets.

Table~\ref{tbl:mostfreq_perf} shows a comparison between the performance
of \pbe and the naive approach {\em MostFreq}.  \pbes performs better
than {\em MostFreq} in 29 out of 40 (i.e., 72.5\%) participant-policy cases,
and for 75\% of the participants.  The average accuracy of \pbes exceeds {\em
MostFreq} (71\% accuracy) as well. 

Note that {\em MostFreq's} accuracy is abysmally low (e.g., 17\%) in
certain cases is due to its over-dependence on the probability
distribution of the training examples. That is, {\em MostFreq} only does
well when the testing dataset consists of examples that are very similar
to the training set as a whole. \pbes does not make any assumptions
about the probability distribution of data, and hence does not suffer
from the same flaw. We discuss the causes of incorrect predictions
(\ref{rq:accuracy-causes}) in Section~\ref{sec:analysis_of_results}.

%% REVIEW (RQ4, RQ5)
% 22 errors identified in manual review
% 100 errors identified in automated review

\subsection{Effectiveness of Active Learning}
\input{review_tbl} 
\begin{comment}
We performed a two-step review process before testing for accuracy,
where we allowed or users to identify and correct incorrect policy
decisions in their examples. First, users performed a manual review of
their examples, for each policy. This was followed by an automated
review using \pbe's conflict resolution approach described in
Section~\ref{sec:algorithm}. 
\end{comment}
We now discuss the effectiveness of \pbe's active learning approach over
manual reviews by participants, for finding labeling errors (i.e.,
errors in the policy decisions of examples) in their specification
datasets.

Table~\ref{tbl:review} shows the number of labeling errors found by the
participant through the manual review, followed by the additional errors
found using \pbe's interactive approach.  The errors found using \pbe's
approach are additional as we used the corrected dataset from the manual
review for the \pbe-assisted review, as described in
Section~\ref{sec:experiments}.

%Table~\ref{tbl:review} shows the number of labeling errors found by the
%participant through the manual review, followed by (i.e., indicated by
%$\rightarrow$) those found using \pbe's interactive approach. \pbe's
%review is carried out using the corrected data from the manual review,
%hence the errors identified are in addition to the ones identified in
%the manual review. 

First, we observe at least one labeling error in most participant-policy
cases, i.e., in 30 out of 40, or 75\% cases. Out of 1,230 total examples
in the specification dataset, we observe 96 total errors (i.e., about
7.8\%) (\ref{rq:user-error}). While participants identify some errors
manually, \pbe's semi-automated process helps the participant identify
and correct the maximum number of errors (80 out of 96, or about 83\%).
For all 8 participants, the total errors (across policies) found by
\pbes are equal to or more than the participant's manual review. Thus,
we conclude that while participants make some error (average 7.8\%)
(\ref{rq:user-error}), participants find more errors using \pbe's
interactive approach than by themselves(\ref{rq:user-error-auto}).
%\pbe's active learning approach is more effective at finding errors than a manual-review
%(\ref{rq:user-error-auto}).

We note that \user{1} did not find any errors manually, nor did
they agree to \pbe's recommendations as they had confidence in their
examples. Further, our accuracy is also the highest for \user{1} as seen
in Table~\ref{tbl:coinflip_perf}. However, given the absence of any
trend in other cases, we refrain from claiming any relation between the
user errors found in the reviews and accuracy.

%Finally, we observe that no errors were detected for User 1, who also
%scores the highest accuracy for our approach across all policies.
%Unfortunately, this trend, or any conclusive relationship, cannot be
%drawn between the errors and accuracy for other users. Hence, we assume
%this interesting occurrence as an outlier.


==> policy-example.tex <==
%\subsection{The Structure of a Policy Example}
%\label{sec:policy-example}
A {\em policy example} $P$
is composed of 1) the {\em policy label} $l$ (i.e., the ``what''), which
describes the resource to be protected or the conditions that influence
the particular policy decision, and 2) the {\em policy decision} $d$
(i.e., the ``how''), which we assume to be a binary decision (i.e.,
allow/deny) for simplicity.  A label is a set of of {\em tags} $t$,
which may be opaque identifiers that mark the inclusion of specific
conditions relevant to the policy, drawn from a universal set of tags
$U$.  A policy rule $P_i$ can be described with
Equation~\ref{eqn:policy-example}.
\begin{multline}\label{eqn:policy-example}
\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ P_i = <l_i, d_i>,\\
%P_i = <l_i, d_i>,\\
    where\ l_i = \{t | t \in U\}
\ and\ d_i\in \{ALLOW,DENY\}
\end{multline} 

Our approach hinges on the findings of a study performed by Klemperer et
al.~\cite{klms+12}, which demonstrates that tags created for organizing
data can be effectively re-purposed to express express access control
policies. Such tags are often available through applications. For
example, Google Maps allows the user to tags certain frequent locations
(e.g., Home, Work) for convenience. Further, Google Keep and EverNote
provide predefined tags (e.g., Work, Grocery) for their notes, and also
allow users to create new tags. We extend this idea of using tags by
allowing users to combine tags into labels to express complex situations
where more than one tag may apply. As a result, a label can also be
thought of as a conjunction of tags, rather than a simple set.

%A label may represent a combination of security-related conditions,
%protected operations on user data, or even indicate the presence of
%sensitive classes of information.  

In this paper, we study the specification of data secrecy policies as an
application of our approach. In the case of data secrecy policies for
application data, the tags are user or application-defined information
classes (e.g., receipts, data created at the Hospital), and the label on
a data object describes all the classes of information that the data
object is derived from.  For example, Alice's security preference of not
having receipts created at the hospital synced with the cloud (discussed
in Example 1 (Section~\ref{sec:motivation}) can be specified using the
following policy example:  

\noindent
{\small
\begin{center}
{\tt label=}``receipt'' $\wedge$ ``hospital'', {\tt decision=}``DENY''
\end{center}
}
%\vspace{0.25em}
\subsubsection{Policy Examples for Bob}
\label{sec:running-example}
\begin{table}[t]
\footnotesize
\centering
\caption{Bob's examples for the {\em WorkCloud} policy.}
%\vspace{-0.5em}
\label{tbl:bob-policy}
\begin{tabular}{l|c|c}
  \Xhline{2\arrayrulewidth}
  {\bf No.} & {\bf Label}             & {\bf Policy Decision}\\
  \Xhline{2\arrayrulewidth}
  1 & Home$\wedge$Photo   & DENY  \\
  2 & Work$\wedge$Photo   & ALLOW  \\
  3 & Photo   & DENY  \\
  4 & Document & ALLOW \\
  %4 & Home $\wedge$ Document & DENY \\
  \Xhline{2\arrayrulewidth}
    \end{tabular} 
\end{table} 

For better understanding, we describe a simple policy specification by
Bob, for a policy designed to control the export of data to the
enterprise cloud, i.e., the {\em WorkCloud} policy. Bob specifies policy
examples using two kinds of tags: 1) Tags that indicate the location of
data creation (e.g., ``Work'' and ``Home'') and 2) tags that indicate
the class or type of secret information (e.g., ``Document'' and
``Photo'').  We assume tags to be provided by applications used to
create the data (e.g., Keep) or the operating system on the smartphone.
Note that applications often provide users with tags to organize data,
which may also be leveraged for specifying security policies.

Bob creates the policy examples shown in Table~\ref{tbl:bob-policy}. Bob
does not work after work hours, and Bob's objective is separate work and
personal data. Therefore, Bob denies export for personal photos created
at home (example 1), although he allows export for photos created at
work (example 2). Further, Bob is conservative about photos that may be
created at an untagged location (example 3), hence export is denied for
such photos.  At the moment, Bob does not imagine a situation where he
would deny export for data created or scanned as documents. Hence, Bob
allows documents to be exported (example 4).

%Now consider a new runtime scenario wherein Bob creates a document at
%home. What policy decision should the system enforce for this new label
%{\tt Home$\wedge$Document} ? The \pbes approach answers this exact
%question, using the algorithm described in Section~\ref{sec:algorithm}.

% Scope
Finally, we note that our policy example format is generic, and is
independent of the actual action/operation controlled by the policy. The
operation controlled by the policy (e.g., exporting data to the cloud)
is a feature of the policy design, and is independent of the problem of
policy specification. The policy format described in this section may be
used for policies that enforce a binary decision and which can be
expressed using a conjunction of conditions. We discuss some
applications of our approach in Section~\ref{sec:applications}.



==> terms.tex <==
\subsection{Terms}
\label{sec:terms}
\begin{figure}[t]
    \centering
    \includegraphics[width=3in]{figs/terms}
    \caption{The structure of a context-policy example.}
    \label{fig:terms}
\end{figure} 

Figure~\ref{fig:terms} describes the anatomy of a policy example. A {\em
policy example} is composed of a {\em label}, and a policy {\em
decision}.  A label is a conjunction of {\em tags}, opaque identifiers
that mark the inclusion of specific user resources relevant to the
example. For instance, in the case of a data secrecy policy for
application data, the tags are user or application-defined information
classes (e.g., Receipts, data created at the Hospital).  For simplicity,
we assume the policy decision to be binary, i.e., allow or deny.  Note
that the operation controlled by the policy (e.g., read, write) is a
part of the policy definition, and is independent of the policy example.

\begin{lstlisting}[basicstyle=\ttfamily\scriptsize,float,caption={Policy
  examples to represent secrecy
  policies},belowcaptionskip=-6mm,label=lst:policy_example,emph={decision,label},emphstyle=\bfseries]
//Scenario 1: Export all receipts, except medical.
$e_1$. label= receipt : decision = ALLOW
$e_2$. label= receipt ^ hospital : decision = DENY
\end{lstlisting}

Consider the motivating scenarios described in
Section~\ref{sec:motivation}. Each scenario can be described using a set
of policy examples. For instance, Listing~\ref{lst:policy_example} uses
two policy examples $e_1$ and $e_2$ to express the first scenario where
Alice wants to export all receipts to the cloud, except receipts taken
at the doctor's office or hospital. The tags $receipt$ and $hospital$
are information classes created by applications (e.g., Evernote), that
denote data saved as a receipt and data created at the hospital
respectively.

